AdvFusion: Adapter-based Knowledge Transfer for Code Summarization on Code Language Models

Programming languages can benefit from one another by utilizing a pre-trained model for software engineering tasks such as code summarization and method name prediction. While full fine-tuning of Code Language Models (Code-LMs) has been explored for multilingual knowledge transfer, research on Parameter Efficient Fine-Tuning (PEFT) for this purpose is limited. AdapterFusion, a PEFT architecture, aims to enhance task performance by leveraging information from multiple languages but primarily focuses on the target language. To address this, we propose AdvFusion, a novel PEFT-based approach that effectively learns from other languages before adapting to the target task. Evaluated on code summarization and method name prediction, AdvFusion outperforms AdapterFusion by up to 1.7 points and surpasses LoRA with gains of 1.99, 1.26, and 2.16 for Ruby, JavaScript, and Go, respectively. We open-source our scripts for replication purposes.

==> Sections/Experiments.tex <==
\subsection{Backbone Models} \label{sec:backbones}

We have selected CodeBERT\cite{feng2020codebert} and GraphCodeBERT\cite{guo2020graphcodebert} as our baseline models for several reasons. These models have been extensively researched in the field of software engineering~\cite{ahmed2021multilingual,saberi2023model,lu2021codexglue,wang2023oneAdapter,chung2014empirical}.
Additionally, these models are studied for multilingual fine-tuning for these two tasks and therefore can be a basis for our comparisons \textcolor{red}{[CITE]}. 

\textcolor{red}{you might add sth about why CodeT5 is not used. there is a paper mentions that multilingual fine-tuning for codet5 does not work. I am not sure how to mention it now, but, we need to reason about not using CodeT5 to answer reviewer2!!}

\textcolor{red}{ADD THE EXPLANATION ABOUT CODE-LMS VS LARGER CODE-LLMS AND CITE HERE. EXPLICITLY MENTION THAT FOR THIS REASON, WE FOCUS ON THESE TWO SMALLER MODELS.}

% We have observed the rise of powerful Large Language Models (LLMs) like CodeLlama \cite{code-llama-roziere2023code}, AlphaCode \cite{alphacode-li2022competition}, and StarCoder \cite{li2023starcoder}, tailored for complex tasks such as competition-level code generation. However, our focus is on smaller models suited for lighter tasks like code summarization and method name prediction. We aim to utilize multilingual knowledge transfer in these models, envisioning them as accurate plug-ins across different Integrated Development Environments (IDEs), addressing specific needs within software development efficiently.

% In contrast, we have observed the emergence of code Large Language Models (LLMs) like CodeLlama\cite{code-llama-roziere2023code}, AlphaCode\cite{alphacode-li2022competition}, and StarCoder\cite{li2023starcoder} in recent years. However, it is essential to note that these LLMs are designed for more complex tasks. For instance, AlphaCode\cite{alphacode-li2022competition} is a competition-level code generation model. Our focus, however, is on leveraging multilingual knowledge transfer in smaller models tailored for lighter tasks, such as code summarization and method name prediction.
% We envision using these smaller models as plug-ins for method name prediction with high accuracy across various Integrated Development Environments (IDEs). This approach aligns with our motivation to apply multilingual knowledge transfer in a practical and efficient manner, addressing the specific needs of lighter target tasks within the software development domain.



\textbf{CodeBERT}, as introduced by \citet{feng2020codebert}, is a bimodal pretrained model designed for both natural language and programming language understanding. Its architecture is based on Transformers. CodeBERT employs two pre-training objectives, namely Masked Language Modeling and Replaced Token Detection. These objectives are specifically chosen to enhance its capabilities in supporting tasks such as code search and code documentation generation.

\textbf{GraphCodeBERT}, introduced by \citet{guo2020graphcodebert}, is a pioneering pre-trained model designed to enhance code comprehension tasks such as code summarization. GraphCodeBERT utilizes semantic-level information from code, specifically focusing on aspects like data flow. This pre-training approach employs a 12-layer transformer-based architecture. It is pre-trained on Masks Language Modeling, Edge Prediction and Node Alignment objective functions.

\subsection{Tasks}
\subsubsection{Code Summarization} \label{sec:task1}

Given a code snippet, the task of code summarization is to describe its functionality. 
\textcolor{red}{Add more explanation about this task and its importance. So reason about why we selected it.}
% In RQ1 and RQ2, the experiments are conducted on monolingual and multilingual datasets, respectively. 
% For monolingual dataset settings (RQ1), RoBERTa \cite{zhuang2021robustly}, CodeBERT \cite{feng2020codebert}, GraphCodeBERT \cite{guo2020graphcodebert}, and CodeT5 \cite{wang2021codet5} are considered. 
% For multilingual dataset settings (RQ2), we compare the results with \textit{Polyglot}GraphCodeBERT \cite{ahmed2021multilingual} and \textit{Polyglot}CodeBERT \cite{ahmed2021multilingual}, as these are the only models that are fine-tuned on multilingual dataset. 
% \textit{Polyglot}GraphCodeBERT fine-tunes GraphCodeBERT \cite{guo2020graphcodebert} on the multilingual dataset from CodeSearchNet, while \textit{Polyglot}CodeBERT fine-tunes CodeBERT \cite{feng2020codebert} on the multilingual dataset from CodeSearchNet.

% The length of the source and target sequences in our setting are 256 and 128, respectively. We set the learning rate to $10e-5$, and batch size to 64 for the fine-tuning phase in all experiments. 

\textbf{Evaluation metric}
We evaluate the code summarization task using \textcolor{red}{smooth-bleu-4???}BLEU \cite{papineni2002bleu}, which is a widely used metric in natural language generation tasks and many software engieering studies \textcolor{red}{[CITE a few papers]}.
% ,
% and provide a way to compare the generated summaries against the ground truth comments. 
BLEU is a precision-based metric that measures the n-gram geometric precision between the generated summary (i.e., n-gram hit) and the ground truth summary (i.e., total n-gram count) \cite{papineni2002bleu}.
\textcolor{red}{Although there are research about the weaknesses of BLEU score for code summarization [CITE], we should this metric because ?????. Also, as the results are all reported in the same metric, it is a fair comparison and will not threat the validity of the results.}

% In this work, we computed the smoothed BLEU-4 score as introduced in \cite{lin2004orange} {where one count is added to the n-gram hit and total n-gram count for $n>1$.}
% For calculating BLEU-4 score we first measure the brevity penalty factor (BP) as follows:

% \begin{equation}
%   BP =
%     \begin{cases}
%       1 & \text{if $c > r$}\\
%       e^{1-r/c} & \text{if $c \leq r$ }\\
%     \end{cases}       
% \end{equation}


% where $c$ is the length of the candidate translation and $r$ is the effective reference corpus length. Next, we calculate the geometric mean of the adjusted precision scores for the test corpus, and then we multiply this outcome by the brevity penalty factor ($BP$) in the following fomula:

% \begin{equation}
%   BLEU = BP.exp \big( \sum_{n=1}^N w_n \text{log} P_n \big)   
% \end{equation}


% Here, $P_{n}$ is the geometric average of the n-gram precision, using n-grams up to length $N$ and $w_{n}$ is the positive weights summing to one.





% \textcolor{red}{Still remaining:
% 2) Why newer models such as CodeT5 and CodeX are not considered ? We may skip this one and leave it for revisions! 3) Why only two tasks, which are basically both code summarization chosen here? You are proposing a general architecture and you claim it works generally for knowledge transfer among various PL, but you only limit it to one task. At this point, do not add anything to it. I think we should change the work to knowledge transfer for code summarization. See the title too. Let me know your thoughts on this. }


% Though these models do not achieve the state-of-the-arts results in code summarization, they are the only models that are fine-tuned on multilingual dataset, and still they have comparable BELU scores with the recent pretrained models for this task. Therefore, we use as our baselines for RQ2. 

% \noindent \textbf{CodeT5} \cite{wang2021codet5} pretrains T5 \cite{raffel2020exploring} on masked span prediction, identifier tagging and masked identifier prediction objective functions using CodeSearchNet data.

% \noindent \textbf{ProphetNet-X} \cite{qi2021prophetnet} is a large-scale pre-trained encoder-decoder model for different languages, downstream tasks and domains. ProphetNet-Code refers to the finetuned model for code summarization on CodeSearchNet dataset.

% We compare CodeBERT + AdvFusion, and CodeBERT + Fusion with these models, as all of them use the same dataset.





% We choose CodeBERT \cite{feng2020codebert} and $polyglot$CodeBERT \cite{ahmed2021multilingual} as our baseline models, both of them are trained on CodeSearchNet dataset \cite{husain2019codesearchnet}. CodeBERT is a multilingual pretrained model finetuned on monolingual datasets, and $polyglot$CodeBERT is a multilingual pretrained model finetuned on multilingual languages. 
 

% \textcolor{red}{Explain what smooth blue is!}








\subsubsection{Method Name Prediction} \label{sec:task2}

 The objective of the method name prediction task is to generate the most fitting method name that describes the purpose and functionality of the method's code. For our experiments, we selected CodeSearchNet as our experimental dataset, as outlined in the study by Husain et al. (2019) \cite{husain2019codesearchnet}. Prior to our work, Jain et al. (2020) conducted an experiment on predicting method names, but this was limited to a subset of JavaScript language samples from CodeSearchNet \cite{jain2020contrastive}.


% In addition to our primary experimental framework, we incorporate CodeBERT \cite{feng2020codebert} and GraphCodeBERT \cite{guo2020graphcodebert} as the backbone models. So one time we fully fine-tune these models on our dataset. The next time we fine-tune them using task adapters to answer the first research question (RQ1). Our focus in this specific task is centered on addressing the second research question (RQ2), which seeks to evaluate the impact of leveraging insights from different programming language structures when predicting method names within a target language context. This investigation aims to shed light on how the incorporation of cross-language latent knowledge can enhance the accuracy and performance of method name prediction. 

In addition to our primary experimental framework, we use CodeBERT \cite{feng2020codebert} and GraphCodeBERT \cite{guo2020graphcodebert} as backbone models. We fully fine-tune these models on our dataset and also fine-tune them using task adapters to address RQ1. Our focus for this task is on RQ2, which evaluates the impact of using insights from different programming languages to predict method names in a target language. This aims to show how cross-language knowledge can improve prediction accuracy and performance.

\textbfn{Evaluation metric}
We report precision, recall and F1-score for the generated method names. F1 Score is the weighted average of Precision and Recall: $F1 = \frac{2 \cdot (P \cdot R)}{P + R}$. 
Where P and R stands for Precision and Recall, respectively.
% Here, P stands for Precision, and it is computed as $P = \frac{TP}{TP+FP}$, whereas R is the Recall and it is calculated as $R = \frac{TP}{TP+FN}$. P represent the precision, calculated as the length of the intersection of ground truth tokens and generated output tokens (i.e., TP) divided by the length of output tokens (i.e., TP + FP). Similarly, let R represent the recall, calculated as the length of the intersection of ground truth tokens and generated output tokens (i.e., TP) divided by the number of ground truth tokens (i.e., TP + FN).


 
% \subsection{Code Search}
% Given a natural language as an input, the aim is to find the most semantically related code from a set of candidate codes. The length of the natural language and code in our setting is 128 and 256, respectively. We set the learning rate to $2e-5$, and batch size to 32 for the fine-tuning phase in all experiments. 



% \subsubsection{Baseline Models}

% In RQ1 and RQ2, the experiments are conducted on monolingual and multilingual datasets, respectively. Different baseline models on evaluating monolingual and multilingual dataset settings are used due to the nature of the models. For example, the model, CodeBERT, was reported on monolingual dataset settings and thus, we only include it into our baseline models for benchmarking monolingual datasets \cite{feng2020codebert}. 
% For monolingual dataset settings (RQ1), seq2seq \cite{sutskever2014sequence}, Transformer \cite{vaswani2017attention}, RoBERTa \cite{zhuang2021robustly}, CodeBERT \cite{feng2020codebert}, GraphCodeBERT \cite{guo2020graphcodebert}, PLBART \cite{ahmad2021unified}, ProphetNet-Code \cite{qi2021prophetnet}, and CodeT5 \cite{wang2021codet5} are considered. 
% For multilingual dataset settings (RQ2), we compare the results with \textit{Polyglot}GraphCodeBERT \cite{ahmed2021multilingual} and \textit{Polyglot}CodeBERT \cite{ahmed2021multilingual}, as these are the only models that are finetuned on multilingual data. 
% \textit{Polyglot}GraphCodeBERT fine-tunes GraphCodeBERT \cite{guo2020graphcodebert} on multilingual dataset from CodeSearchNet. 
% And \textit{Polyglot}CodeBERT fine-tunes CodeBERT \cite{feng2020codebert} on multlingual data from CodeSearchNet.




% \begin{table*}[t!]
% \centering
% \begin{tabular}{c | c | c| c| c| c| c} 
%  \hline
%  model &  ruby   &  javascript  & go & python  & java &  php \\
%  \hline
%  NBow & 0.162 & 0.157 & 0.330 &  0.161 & 0.171 & 0.152 \\ 
%  CNN & 0.276 & 0.224 & 0.680 & 0.242 & 0.263 & 0.260   \\ 
%  BiRNN  & 0.213 & 0.193 & 0.688 & 0.290 & 0.304 & 0.338 \\ 
%  selfAtt & 0.275 & 0.287 & 0.723 & 0.398 & 0.404 & 0.426 \\ 
% \hline
%  RoBERTa & 0.587 & 0.517 & 0.850 & 0.587 & 0.599 & 0.560 \\ 
%  RoBERTa (code) & 0.628 & 0.562 & 0.859 & 0.610 & 0.620 & 0.579 \\ 
%  CodeBERT & 0.679 & 0.620 & 0.882 & 0.672 & 0.676 & 0.628  \\ 
%  GraphCodeBERT & 0.703 & 0.644 & 0.897 & 0.692 & 0.691 & 0.649  \\ 
% \hline
% GraphCodeBERT + Fusion  & 0.736 & 0.605 & 0.8446 & 0.619 & 0.644 & 0.570  \\
% GraphCodeBERT + AdvFusion  & 0.757 & 0.611 &  0.863 & 0.6314 & 0.654 & 0.591  \\
% %    Number of Parameters  & 124M & 21M  \\
% % \hline
% \end{tabular}
% \caption{code search target task}
% \label{table:task-adapter}
% \end{table*}









% The goal is to evaluate the learned knowledge of programming languages in a pre-trained language model on a low resource programming language using adapters.
% The aim of this research is to extract desirable embeddings from high resource programming languages to fine-tune a pretrained model on a low resource programming language. 



\section{Experiment Setup} \label{section:experiments}
% In this section, we describe the dataset, the model training, baseline models, and the evaluation metrics.

In this study, we assess the effectiveness of our methodology across two code-oriented target tasks, namely, code summarization and method name prediction. To facilitate the application of our approach to these tasks, we emphasize the necessity of training language adapters. All experiments are conducted on an Nvidia Tesla V100 32GB GPU.


\subsection{Language Adapter Training}

As Pfeiffer et al. has performed an extensive hyperparameter search over adapters, we use their reported optimal settings in our adapters' hyperparameters \cite{pfeiffer2020adapterfusion}.

\label{subsec:dataset}
 We use CodeSearchNet \cite{husain2019codesearchnet} for training language adapters. It consists of 6 programming languages and the size of each language is shown in Table \ref{table:plm}. We only use the bimodal dataset for our experiments.


% \begin{table}[h!]
% \centering
% \begin{tabular}{|c | c |} 
%  \hline
%  Language & bimodal Data  \\ [0.5ex] 
%  \hline
%  Ruby  & 24,927  \\
%  \hdashline
%  JavaScript  & 58,025  \\
%  Go  & 167,288  \\ 
%  \hdashline
%  Python  & 251,820  \\ 
%  Java  & 164,923  \\ 
%  PHP  & 241,241 \\ 
%  \hline
% \end{tabular}
% \caption{Dataset used for training PLM \cite{husain2019codesearchnet}}
% \label{table:plm}
% \end{table}


\begin{table}[h!]
\centering
   
    \begin{tabular}{|c | c | c| c|} 
        \hline
        Language & \# of Bimodal Data & Language & \# of Bimodal Data \\ [0.5ex] 
        \hline
         Ruby  & 24,927  & Python  & 251,820\\
         JavaScript  & 58,025  & Java  & 164,923\\
         Go  & 167,288  & PHP  & 241,241 \\ 
         \hline
    \end{tabular}
    \caption{Dataset statistics.  \cite{husain2019codesearchnet}}
    \label{table:plm}
  
\end{table}





\subsection{Experiments Design}

% Our study explored two tasks, code summarization and method name prediction. We note that our main objective is to aggregate the latent knowledge from different programming languages, and to achieve that, we opted for the CodeSearchNet dataset (\cite{husain2019codesearchnet}) due to its inherent diversity (it consists of six different programming languages) as detailed in Section \ref{subsec:dataset}. Furthermore, it has been widely used in previous studies \cite{feng2020codebert, wang2021codet5, ahmed2021multilingual, guo2020graphcodebert}.
% Our backbone models consist of CodeBERT (\cite{feng2020codebert}), and GraphCodeBERT (\cite{guo2020graphcodebert}). We applied the task of code summarization and method name prediction to both of them. The details about choosing these models and the explantion of the tasks are discussed in Sections \ref{sec:backbones}, \ref{sec:task1}, and \ref{sec:task2}.

Our study delves into code summarization and method name prediction tasks, aiming to gather diverse programming language knowledge. We utilized the CodeSearchNet dataset for its six-language diversity, widely adopted in prior research (\cite{husain2019codesearchnet}). Our backbone models, CodeBERT (\cite{feng2020codebert}) and GraphCodeBERT (\cite{guo2020graphcodebert}), were employed for both tasks. The details about choosing these models and the explanation of the tasks are discussed in Sections \ref{sec:backbones}, \ref{sec:task1}, and \ref{sec:task2}.



% To conduct our study, the dataset and downstream task chosen are CodeSearchNet, which consists of six programming languages (Section \ref{subsec:dataset}), and code summarization, respectively. Code summarization refers to generating natural language description for a given code snippet \cite{zhang2022survey}. Code summarization is chosen as it enables us to evaluate the model's generation ability while focusing on both natural language and programming language modalities of the model and this task is used in multiple studies \cite{wang2021codet5,feng2020codebert}.
% % We choose code summarization as it is \textcolor{red}{EXPLAIN THE REASON.}
% To conduct our experiments, we choose CodeBERT \cite{feng2020codebert} as the backbone model to insert adapters.
%  CodeBERT is selected as it is used in numerous software engineering studies previously \cite{ahmed2021multilingual,chen2022transferability,ahmed2022few}.
%  Though CodeT5 has the state of the arts results, it is not chosen in our experiment, because the pretrained MLM version of CodeT5 is not available online.

% \textbf{RQ1:}
% To address \textit{RQ1}, we fine-tune CodeBERT and GraphCodeBERT for code summarization and method name prediction using task adapters. To accomplish this, we maintained the weights of the code-LMs, integrated the task adapters into CodeBERT and GraphCodeBERT, and fine-tuned them for code summarization and method name prediction. These modified models are denoted as CodeBERT+TaskAdapter and GraphCodeBERT+TaskAdapter. We then compared the performance against the full fine-tuning of CodeBERT \cite{feng2020codebert} and GraphCodeBERT \cite{guo2020graphcodebert} for each programming language.

% \textcolor{red}{We need to change the following based on changing RQ1.}
% As the task adapters and the fine-tuning of the LMs are done on each programming language separately, we refer to this as \textit{monolingual task adapter based fine-tuning}.


 \textbf{RQ1:}
In \textit{RQ1}, we investigate if adapters trained with a multilingual dataset can improve the performance of the down stream task in a specific programming language. We refer to this setting as \textit{multilingual adapter-based fine-tuning}. 

\textcolor{red}{We need to change the following based on changing RQ1.::}

We first evaluate using AdapterFusions, where we learn the latent knowledge from the multiple language adapters for a target language. We refer to these models as CodeBERT+Fusion and GraphCodeBERT+Fusion.

% Although the pre-trained model has knowledge of all the seen programming languages (i.e., the languages used in its pre-training), when we fine-tune all the weights on an imbalanced multilingual dataset, the weights are affected mostly by the high-resource languages. To address this challenge, we adapt a pre-trained model and extend it with a parallel stack of trained language adapters. When a sample is fed into the model, the output of each adapter will be the network embeddings focusing on the corresponding language.



To train AdapterFusion, we first train six language adapters individually that corresponds to each of the programming language in our dataset, while fixing the weights of the LM.
These adapters are trained on the Mask Language Modelling objective to capture the language-specific embeddings that exist in the code-LM. Then, we train an AdapterFusion on top of these language adapters to select the attention from each language adapter. 
AdapterFusion then aggregates the extracted embeddings from all the language adapters of each input. 






In the following, we introduce AdvFusions to enforce the model to learn more from other programming languages. In the first phase, we (1) fixed the weights of the language adapter, (2) temporarily set the weights of the language adapter corresponding to the current input (i.e., the language of the target task) to zero, and (3) trained the weights of the AdvFusion on our target task. In the second phase, we restore the language adapter weights corresponding to the input and allow AdvFusion to learn from the language adapter belonging to the current input.

 % We use our proposed approach, \textit{AdvFusion}, to assess its effect for low resource languages and refer to our model as \textbf{\textit{AdvFusion}CodeBERT} and \textbf{\textit{AdvFusion}GraphCodeBERT}.


We evaluated \textit{AdvFusion} performance on code summarization and method name prediction using both CodeBERT and GraphCodeBERT, refer to as \textbf{CodeBERT + AdvFusion} and \textbf{GraphCodeBERT+AdvFusion}, respectively.



% Language adapters are similar to the task adapters, but differ in the sense that language adapters are trained on MLM while task adapters are trained on an objective of a downstream task. 


% As explained in Section \ref{subsec:architecture}, the fusion adapter has more tendency to pay more attention to the language adapter corresponding to the current input. \cite{pfeiffer2020adapterfusion}. 
% Therefore, we apply our introduced adapter, \textit{AdvFusion} which enforces the model to learn from other programming languages. 

% We introduce AdvFusions to enforce the model to learn more from other programming languages. In the first phase, we (1) fixed the weights of the language adapter, (2) temporarily set the weights of the language adapter corresponding to the current input to zero, and (3) trained the weights of the AdvFusion. At the end of the first phase, we force the model to learn from other languages. In the second phase, we restore the language adapter weights corresponding to the input and allow the model to learn from the language adapter belonging to the current input.




\textbf{RQ3:}
For \textit{RQ3}, we evaluate the contribution of each programming language for a target programming language. Here, we choose Ruby as it has less samples and it could take more advantage of other programming languages. Ruby is used as a low resource language in previous studies~\cite{chen2022transferability}. 

% first plugging a stack of six programming language adapters followed by a fusion adapter on top of them to the pretrained CodeBERT model; all of them were trained previously, (2) 
% The contribution is computed by first feeding the Ruby test dataset to CodeBERT+Fusion. Then, we aggregate all the attention scores from each language adapter in each layer and normalize (i.e., min-max normalization) the aggregated attention to obtain the percentage of each language contribution.
% We repeat the above steps for \textit{AdvFusion}CodeBERT to compare the ability of the AdapterFusion and AdvFusion to extract knowledge from other programming languages for Ruby. We were limited by computational resources, so we conducted attention calculations only for each layer of the CodeBERT model.

We compute contributions by feeding the Ruby test dataset into CodeBERT+Fusion. Then, we aggregate attention scores from each language adapter in each layer, normalize them ( i.e., min-max normalization), and obtain the percentage of each language's contribution. We repeat these steps for AdvFusionCodeBERT to compare its ability with AdapterFusion in extracting knowledge from other programming languages for Ruby. Due to computational limitations, we calculate attention only for each layer of the CodeBERT model.


% \section{Approach}
% \label{section:approach}
% Our approach consists of the following steps:
% \begin{itemize}
% \item  First, we need a component that extracts the embeddings of the trained programming languages that help capture the syntax/semantics of the unseen language. [EXPLAIN WHY USING ADAPTERS]. Although the pretrained model consists of the knowledge of all seen PLs, it needs to select the most similar ones and ignore the irrelevant parts of the seen languages, which are considered as a noise for an unseen language. Adapters are lightweight modules placed on the transformer blocks that allow the model to select the relevant knowledge in each block based on the objective function defined for the network. We take advantage of language adapters trained on an abstract objective function such as mask language modeling to capture the syntax/semantics for each programming language. In this regard, we separately train language adapters for each seen language. If there are six programming languages seen in the pretraining, we will have six language adapters trained separately on the MLM. When an unseen language is fed to the pretrained model extended with a parallel stack of trained adapters, the output of each adapter is the network prediction focusing on a specific seen language.


% \item  In the next step, we need a component that aggregates the relevant embeddings on the adapters' outputs for an unseen language. Fusion adapter has an attention architecture and aims to learn how to pay attention to relevant embeddings of its previous layer. We place a fusion adapter on top of the trained language adapters to select the relevant embeddings from the outputs of the language adapters. Then, We train the fusion adapter on an unseen language and downstream task by freezing the weights of the language adapters and the pretrained model. This approach not only could select the relevant data from each seen language but also for a new unseen language, we do not need to repeat the first step and only train the fusion adapter to reattend in language adapters based on the new unseen language.

% \end{itemize}





% \subsection{Study Design}



% \textbf{RQ1 Design}: We considered multilingual PLMs such as CodeBERT\cite{feng2020codebert} and GraphCodeBERT as our backbone models and code summarization as our downstream task, which are widely used in the literature. We evaluate the performance of adapters by finetuning them on Ruby language, which is a low resource language, and calculate the performance of adapters by designing two experiments:
% \begin{itemize}
%     \item 
%     Backbone models should be finetuned in a standard way, which means taking the pretrained model and finetune the entire weights of the model in the low resource language. This is our baseline model to compare the performance of standard finetuning and adapter-based finetuning.
%     \item
%     We fix the backbone model weights, plug task adapter into the intermediate layers of the model, and train them on the low resource language.
% \end{itemize}

% For each experiment, we consider the total number of training weights and training time as well as the accuracy of the model on code summarization.  

% These experiments aim to show how much improvement could be done by enforcing the weights of the pretrained model to be fixed during the finetuning phase. In NLP, \cite{lee2019mixout} demonstrates that if the model weights stay closer to the initial weights of the pretrained model, we will avoid catastrophic forgetting and stabilize the finetuning process, which leads to accuracy improvement. In this study, we go one step further, fix the pretrained weights, and evaluate the adapter's performance compared with standard finetuning in NL-PL language models.


% \begin{table}[h!]
% \centering
% \begin{tabular}{|c c c c c|} 
%  \hline
%  Method & Ruby & Python & PHP & \# parameters \\ [0.5ex] 
%  \hline\hline
%  CodeT5  & 15.24 & 20.01 & 26.03 & ~220M   \\ 
%  CodeT5 + Task Adapters & 15.20 & 19.89 & 25.92 & 1.7M \\
%  \hline
% \end{tabular}
% \caption{Smoothed BLEU-4 scores on code summarization task.}
% \label{table:comparison}
% \end{table}

% \begin{table}[h!]
% \centering
% \begin{tabular}{|c c c c c|} 
%  \hline
%  Method & Ruby & Python & PHP & \# parameters \\ [0.5ex] 
%  \hline\hline
%  CodeT5  & 15.24 & 20.01 & 26.03 & ~220M   \\ 
%  CodeT5 + Fusion Adapter \\
%  (Ruby, Python, PHP) & 15.52 & 20.47 & 25.92 & 1.7M \\
%  (All) & 15.25 & --  & --  &  -- \\
%  (Ruby, Python) & 15.40 & --  & --  &  -- \\
%  \hline
% \end{tabular}
% \caption{Smoothed BLEU-4 scores on code summarization task.}
% \label{table:comparison}
% \end{table}


% For RQ1, I had an experiment on the CodeT5 model in which I trained an adapter for the code summarization task on python using codesearchnet dataset. In the codeT5 paper \cite{wang2021codet5}, the whole model with 222M parameters was trained and achieved a blue score of 20.36 for this task. This is while, when I applied adapters to the pre-trained CodeT5 model, the total number of trainable parameters decreased to 1.7M parameters and the mode achieved the blue score of 19.89. This decline in accuracy makes sense because we trained a very small subset of parameters and based on the adapter's main paper, they experienced the same manner in the NLP tasks\\


==> Sections/Introduction-old.tex <==
\section{Introduction}\label{sec:introduction}
% \section{Introduction}
\label{section:introduction}
% \textcolor{red}{Problem introduction}

% Researchers have shown that training multilingual models can improve the performance for low resource languages (i.e., languages with small datasets) in downstream tasks \cite{dabre2020survey,ranathunga2021neural,ha2016toward,tang2020multilingual}. 


% \textcolor{red}{Needs a coonection.}
% \fuxiang{Maybe this sentence is redundant?} 


Providing high-quality large datasets is a challenging and time-consuming activity \cite{otter2020survey, ahmed2021multilingual,chen2022transferability,2020arXiv200809824S}. 
Inspired by the success of using Pre-trained Language Model (PLM) in transfer learning for low-resource languages (i.e., a language that is lacking training data) in Natural Language Processing (NLP) \cite{dabre2020survey,ranathunga2021neural,ha2016toward,tang2020multilingual}, several Natural Language to Programming Language (NL-PL) models were proposed to take advantage of high-resource (i.e., a language that has abundance of training data) datasets for tasks involving low-resource programming languages \cite{ahmed2021multilingual,chen2022transferability,ahmed2022learning}.

% Models trained on both source code and natural language are not an exception and low resource dataset makes the model suffer from overfitting.

% Recently, several studies have been conducted on transferring the knowledge of high resource programming languages to a low resource target language in the software field \cite{ahmed2021multilingual,chen2022transferability}.

Multilingual fine-tuning is to fine-tune a PLM with datasets of different languages, and a multilingual PLM is a language model pre-trained on different languages. \citet{ahmed2021multilingual} reported that fine-tuning a multilingual code-based PLM (e.g., PolyglotCodeBERT and PolyglotGraphCodeBERT) on CodeSearchNet \cite{husain2019codesearchnet}, a multilingual dataset consisting of six programming languages (i.e., Ruby, JavaScript, Go, Java, Python and PHP), yields better results on code-related tasks such as code summarization, code retrieval, and method name prediction, as compared to fine-tuning a multilingual PLM on a monolingual dataset. 
% \fuxiang{Are we going to use identifiers in our work somewhere? If no, can we omit this sentence?} This is mainly due to the fact that identifiers play an important role in training a model and also programmers use similar identifiers in different Programming Languages (PLs). 
However, there are semantic and syntactic differences among different programming languages \cite{chen2022transferability} and training a PLM on several different programming languages can lead to knowledge interference -- the same semantic has different syntax or the same syntax has different semantic in different programming languages, and mixing them can cause confusion in learning. For example, Python employs an indentation-based code structure while Java uses parenthesis for separating blocks; and the \verb |default| keyword has a different meaning in Java than it has in Go \cite{zhang2022survey}. If we combine them together, it may confuse the model's learning process.


% On the other hand, \citet{pfeiffer2020unks} shows that due to limited capacity of multi-lingual models and imbalanced datasets, there is a performance gap between high resource and low resource languages

In a separate study, \citet{chen2022transferability} analyzed the transferability of code-based PLMs for Ruby, a low-resource language, for two downstream tasks: code summarization and code search. It was reported that for the target programming language, Ruby, the PLMs that were pre-trained on programming languages similar to Ruby yield better performance on the downstream tasks. They also proposed a strategy to select similar programming languages for pre-training a PLM based on the semantic and textual similarities of the target programming language . 

The former study \cite{ahmed2021multilingual} utilized the entire dataset and did not consider the syntactic and semantic differences of various programming languages, which may cause knowledge interference, while the latter work \cite{chen2022transferability} mitigates this knowledge interference by selecting only a subset of dataset for training that are similar to the \textit{target} programming language.
The other datasets that were not selected for training, howerever, can still be useful due to their high-resource nature and there could still be other useful latent similarities. Thus, we would like to better utilize the entire dataset  (i.e., multilingual dataset) by selecting only the \textit{similar aspects} of each programming language in the dataset for a \textit{target} programming language. In this paper, the primary objective is to investigate whether tailoring training parameters for each language in a multilingual setting can mitigate knowledge interference, and the proposed research question is to explore the impact of employing distinct sets of parameters for each language in a multilingual context.
% EXPLAIN THE CHALLENGE. I.E. WHAT IS THE ISSUE WITH THIS APPROACHES?




% EXPLAIN THE CHALLENGE. I.E. WHAT IS THE ISSUE WITH THIS APPROACHES?

In our study, we leverage pluggable modular components in our model to utilize the entire mulilingual dataset while minimizing the interference among different programming languages.
Modular components have an extensive history in NLP \cite{andreas2016learning,pfeiffer2020adapterfusion,pfeiffer2020mad}. A recently introduced modular component is \emph{adapter}, which is a light-weight module inserted between the Transformer layers \cite{houlsby2019parameter}. It is proposed as a parameter-efficient and quick fine-tuning (i.e., using less number of parameters and less time) approach for fine-tuning Transformer-based models \cite{houlsby2019parameter}.
Adapters have been used previously to show the transferability of natural language PLMs to programming languages with lower training costs~\cite{goel2022cross}. 
% -- the authors trained two different types of adapters, language adapters (i.e., adapters trained on masked language modeling on unlabelled data) and task adapters (i.e., adapters trained for a target task on labelled data) for the code clone detection task \cite{goel2022cross}. 

Although adapters are used previously for transferability of natural languages to programming languages~\cite{goel2022cross}, imposing syntactical information to the pre-trained programming language models~\cite{saberi2023model} and for empirical studies of multilingual fine-tuning~\cite{wang2023oneAdapter} in software engineering, little is known about how adapters can be used for knowledge aggregation for programming languages, nor how adapters can be effectively inserted into the layers of code-based PLMs such as CodeBERT~\cite{feng2020codebert} for fine-tuning downstream tasks. In this work, we focused on the studying of two popular code-related tasks, namely code summarization and method name prediction, and we fine-tuned each of the programming languages in the CodeSearchNet dataset using a multilingual setting through adapters. %in CodeSearchNet dataset \cite{husain2019codesearchnet}.
First, we evaluate if task adapters trained on monolingual data on a code-based PLM can improve the performance of downstream tasks. 
to evaluate to what extent we can leverage adapters for fine-tuning on  and how much performance improvement we can achieve without adding additional data (RQ1). Then, we evaluate specific type of adapter known as \textit{adapter fusions}~\cite{pfeiffer2020adapterfusion}
for aggregating the useful latent information from the multilingual dataset. The process of  aggregation involves leveraging the similar latent information from diverse programming languages to enhance the overall understanding and performance for a specific programming language. With the increasing availability of multilingual data, it becomes crucial to develop techniques that can effectively utilize this wealth of information. Adapter fusions have emerged as a promising solution in this regard. Finally, we propose \textbf{Adversarial Fusion adapter (AdvFusion)} to address the shortcomings of the fusion adapters, as detailed below (RQ2). {In additon, we evaluate the parameter and time efficiency of our fine-tuning approach to the traditional way of  fine-tuning a model.}


We first evaluate to what extent we can improve the performance of monolingual fine-tuning of code-based PLMs using task adapters on code summarization in terms of time and accuracy. We observe that using task adapters for code summarization on Ruby, we achieve an improvement of 16\%, without including data from other languages. 
Based on this result, we leverage language adapters to train language-specific modular components for each programming language on \textit{multilingual} setting to extract knowledge from available languages in the dataset. Each language adapter is trained on a single programming language. 

Next, we train an adapter fusion, an attention-based adapter proposed in \cite{pfeiffer2020adapterfusion}, placed on top of a stack of language adapters using a multilingual dataset. It's aim is to select a set of embeddings for a specific task from the language adapters (See Fig. \ref{fig:fusion-internal}). More specifically, when an input is passed through the network, we have embeddings of that input from each language adapter, and the adapter fusion will select a set of embeddings that will maximize the objective function of the downstream task. 
In NLP, adapter fusions are mainly introduced as a \emph{non-destructive task composition} for transfer learning \cite{pfeiffer2020adapterfusion} where we have a stack of task adapters trained on different downstream tasks, and the adapter fusion will extract a set of embeddings for a particular low-resource language downstream task. 
% In a part of this work, \textbf{we proposed AdvFusion, a variant of the fusion adapters for knowledge extraction from different programming languages and showed that our approach improves the performance for low-resource languages and decreases the fine-tuning computational cost for all languages}.

However, when trained on a particular target language downstream task, the adapter fusion will tend to activate on the same language adapter more at every layer \cite{pfeiffer2020adapterfusion}. For example, given that the downstream task is for a particular programming language, Ruby, and there are two language adapters trained on two different programming language datasets, Ruby and Java. The adapter fusion sits on top of the language adapters and the adapter fusion will pay more attention to the Ruby language adapter than the Java language adapter. In this case, there will be minimal learning from the Java language adapter.
% if we have a {Ruby} sample and our model consist of {Ruby} and Java language adapters as well as an adapter fusion on top of them, adapter fusion tends to pay more attention in {Ruby} rather than Java language adapter, thus, not learning from Java. 
Therefore, \textbf{we propose a variant of the adapter fusion, Adversarial Fusion adapter (AdvFusion),  for knowledge extraction from the different programming language adapters and we show that our approach improves the performance of downstream tasks involving low-resource languages and decreases the fine-tuning computational cost for all languages}.
AdvFusion 
%\fuxiang{Where did this thing comes from? Did you mention it above?} 
enforces the fusion layer to learn more from the other languages for a given target language of a downstream task, instead of focusing on learning from the language adapters, which may cause bias on the language adapter that has the same language as the downstream task. 
We fine-tune AdvFusion on code summarization in two phases. First, we disable the language adapter that is corresponding to the target language that we expect the model to be fine-tuned on and enforce AdvFusion to learn from the other language adapters on that specific task. For example, for code summarization on Ruby, we disable the Ruby language adapter and train AdvFusion to learn only from the other five language adapters that exist on CodeSearchNet. 
In the second phase, we enable the muted language adapter (i.e., Ruby language adapter in this example) and fine-tune AdvFusion the second time on \textit{all} the language adapters. 
When AdvFusion is applied on the multilingual fine-tuning setting on Ruby, we achieved an improvement of 12\% in BLEU score on code summarization over the non-adapter multilingual fine-tuning approach.
%Performing multilingual training on AdvFusion, the BLEU score (a metric used for evaluation of code summarization) are improved by 12\% and 28\% for Ruby and Go, compared to the multilingual fine-tuning of CodeBERT \cite{feng2020codebert}. Our approach outperforms the state-of-the-art code summarization models in low-resource languages.
%Our approach improves the preformance for a low resource language, as we encourage the model to learn more from other high resource languages in the dataset, which is also shown in the attention analysis in our work. 

%\iman{Given a finetuned model with fusion adapters on code summarization, we performed an attention analysis to check how much knowledge a low-resource language could gain from other programming languages at each transformer layer. In this regard, We fed the Ruby test dataset to the finetuned model and aggregated the attention we got from each language adapter at each fusion layer and calculated the percentage of contribution for each language. We performed a similar approach for Adversarial fusion adapters and compared the contribution of each language in Adversarial fusion adapters and fusion adapters.}


% \cite{lee2019mixout} shows that if we encourage the model weights to be closer to the pretrained model during finetuning, we will achieve better performance. \iman{In the next step, we want to assess to what extent we can improve the performance of finetuning phase on a monolingual downstream task using modular components without adding any additional data}.
% We employ adapters to evaluate the performance of adapting a pretrained multilingual programming model for a specific language on a monolingual dataset. This is an alternative to finetune a multilingual model on a monolingual dataset. We plug adapters into the pretrained model and train adapter weights on code summarization while leaving the pretrained weights frozen. As we fixed pretrained weights during the finetuning phase, we expect performance improvement without including additional data. 

\begin{figure}
\centering
    \scalebox{.8}{
    \input{images/internal_fusion}
    }
\caption{Internal structure of fusion and language adapters. Adapter fusion is placed on top of a stack of trained language adapters. The output of the language adapters are fed to the key and value in adapter fusion and for each query, the adapter fusion will choose a set of weights from the language adapters.}
\label{fig:fusion-internal}
\end{figure}




Overall, this paper makes the following contributions:

\begin{itemize}
% \item Adapter finetuning on monolingual datasets yeilds better results than finetuning the whole model on a monolingual dataset.
\item Evaluating the performance of fine-tuning PLMs using adapters on monolingual programming datasets.

\item Proposed a new adapter, AdvFusion, to address the knowledge interference (caused by the different programming languages) by utilizing and combining different language adapters (for each programming language) in the model. 

%\item Evaluate the contribution of each programming language on code summarization for Ruby.

% \item Proposing Type adapters and a new objective function for training them. 

\end{itemize}



The rest of the paper is organized as follows. In Section \ref{section:background}, we provide an overview of important background information and then introduce our proposed adapter, AdvFusion, in Section \ref{section:approach}. In Section \ref{section:rq} we provide the research questions and the details of our study, followed by the experimental setup in Section \ref{section:experiments}. Results are explained in Section \ref{section:result} and they are further discussed in Section \ref{section:discussion}. Sections \ref{section:related-work} and \ref{section:threat} are dedicated to the related works and threats to validity. Finally, we conclude the paper in Section \ref{section:conclusion}.


% \textbf{Significance of Study:}
% Adapters are meant to be be used as quick and parameter efficient alternative approach to fully fine tuning the whole models' parameters. We show that it in addition to this, they can improve the performance ..

% In this study, we show that adapter-based monolingual finetuning is not only a quick and parameter-efficient approach, but it can improve the performance of low-resource languages; so it can be used as an \textit{alternative approach to the monolingual finetuning phase on low resource datasets in the future}. Besides, We provide insights into how much each programming language contributes to code summarization for a low-resource language. This contribution is a similarity indicator for different programming languages from the finetuned model's point of view. \iman{Using AdvFusion, researchers could determine which datasets are more useful for a low-resource language and leverage them more than the Fusion adapter in practice.}



%\todoblue{THE REST OF THE PAPER}















% Later \citet{he2021effectiveness} demonstrates that for monolingual adaptation, adapterbased fintuning yealds better results in NLP area. This is due to the fact that


==> Sections/Introduction.tex <==
\section{Introduction}\label{sec:introduction}
\label{section:introduction}


% Language Models (LM)--models pre-trained on a large corpora-- have gained a lot of attention in the past few years. In Software Engineering (SE), domain specific LMs such as the ones pre-trained on code, also referred to as code-LMs, have achieved the state-of-the-art results in many SE-tasks e.g., code summarization, bug prediction, program repair, method name prediction, and code search \cite{gu2022assemble,ahmed2022learning,zhang2022survey,guo2020graphcodebert,feng2020codebert}. 
% code-LMs are pre-trained on large corpora of multiple programming languages, and then are fine-tuned on supervised data for a downstream task of interest. 
Language Models (LMs), pre-trained on extensive datasets, have surged in popularity. In Software Engineering (SE), domain-specific LMs, known as code-LMs, trained on code, excel in various tasks like code summarization, bug prediction, and method name prediction \cite{gu2022assemble,ahmed2022learning,zhang2022survey,guo2020graphcodebert,feng2020codebert}. They are trained on diverse programming languages and fine-tuned for specific tasks.



% There are multiple studies that investigate the best approach to fine-tune code-LMs, such as considering mono-lingual or multi-lingual dataset for a downstream task during fine-tuning~\cite{ahmed2021multilingual} and using a dataset of a similar programming language for a target programming language~\cite{chen2022transferability}. 
% There are also many studies discussing how to improve the results of a code-LM for low-resource programming languages (i.e., languages lacking abundant training data)~\cite{ahmed2022learning, chen2022transferability} or investigating other fine-tuning paradigms (i.e., parameter efficient fine-tuning), as fine-tuning all parameters of the LM requires a lot of computational resources~\cite{goel2022cross, pfeiffer2020mad,pfeiffer2020adapterfusion,hu2021lora,rathnayake2022adapter}. 

Multiple studies explore optimal approaches to fine-tune code-LMs, including considerations such as mono-lingual vs. multi-lingual datasets~~\cite{ahmed2021multilingual} and using similar programming language datasets for target languages~\cite{chen2022transferability}. Others focus on enhancing results for low-resource languages~\cite{ahmed2022learning, chen2022transferability}  or alternative fine-tuning methods to address computational resource constraints~\cite{goel2022cross, pfeiffer2020mad,pfeiffer2020adapterfusion,hu2021lora,rathnayake2022adapter}.

% \iman{In recent years, Code-LLMs such as CodeLlama \cite{code-llama-roziere2023code} and StarCoder \cite{li2023starcoder} play a crucial role in development of code intelligence tasks. \citet{maunveiling} conducted a comprehensive investigation on how code-LMs and code-LLMs understand code by employing four probing tasks to assess the syntactic and semantic abilities of these models. They even revealed that code-LMs show superior performance than code-LLMs on identifying syntax characteristics. They mentioned this feature indicates fine-tuning code-LLMs on a target task could be more challenging in code-LLMs than code-LMs which supports the result of the other paper \cite{dou2023towards} whose authors compare the results of code-LLMs and code-LMs on clone code detection and most of the code-LM models outperform code-LLMs in this target task. }




Though there are a lot of studies on using code-LMs in software engineering, there is a gap in bridging the above-mentioned directions: knowledge transfer of multiple programming languages for a target programming language and Parameter Efficient Fine Tuning (PEFT). PEFT approaches are introduced as alternatives to fine-tuning all parameters of the model (i.e., full fine-tuning) as they require less number of parameters and less time, thus, reducing the computational costs of using LMs~\cite{houlsby2019parameter}. On the other hand, full fine-tuning the LM on multiple programming languages helps improve the performance of some code-related tasks, as there are similar aspects in programming languages~\cite{ahmed2021multilingual}. 
However, there is no work in software engineering that benefits from the knowledge transfer among programming languages in parameter efficient fine-tuning paradigm. 
In this research, we specifically focus on PEFT using \emph{Adapters}, light-weight modules inserted between the Transformer layers~ \cite{houlsby2019parameter}.




\iman{
In recent years, Code-LLMs such as CodeLlama \cite{code-llama-roziere2023code} and StarCoder \cite{li2023starcoder} have played a crucial role in the development of code intelligence tasks. \citet{maunveiling} conducted a comprehensive investigation into how code-LMs and code-LLMs understand code. They used four probing tasks to assess the syntactic and semantic abilities of these models. Their study revealed that code-LMs perform better than code-LLMs in identifying syntax characteristics. This finding indicates that fine-tuning code-LMs on a target task could be more effective compared to code-LLMs \cite{maunveiling}. This is further supported by \cite{dou2023towards} , whose comparison of code-LLMs and code-LMs on clone code detection showed that most code-LM models outperform code-LLMs in this task. Given these findings, we aim to exploit the capabilities of code-LMs and propose a quick fine-tuning approach to improve their performance.
}

Previous research has shown that adapters are effective for the transferability of natural language models to programming languages with lower training costs~\cite{goel2022cross}. 
New adapter architectures were also shown to be effective in imposing syntactical information to code-LMs and improving their results compared to fully fine-tuning them~\cite{saberi2023model}. 
Other works include empirical studies of adapters in different settings, including multilingual setting, where a dataset of multiple programming languages is used in fine-tuning the code-LM for downstream tasks~\cite{wang2023oneAdapter}.
Still, studies on adapters are limited in the SE domain, and little is known about how adapters can be used for transferring knowledge from other programming languages to a target programming language, specifically when the dataset size of the target language is small. 

In this study, we first show that when we insert adapters that are trained on a specific task (i.e., code summarization and method name prediction) to a code-LM, we can achieve better or on-par results compared to when we fully fine-tune the model. Noticeably, the training time also reduces by $30\%$ to $34\%$. 
Based on this observation, we explore using adapters trained on different programming languages for aggregating the useful latent information from the multilingual dataset for a task in a target programming language. For this purpose, we use a specific architecture known as \emph{AdapterFusions}~\cite{pfeiffer2020adapterfusion}, which leverages similar latent information from diverse programming languages to enhance the performance for a specific programming language of the target task.

% This study demonstrates that integrating task-specific adapters into a code language model can yield improved or comparable results compared to full fine-tuning, with a notable reduction in training time by 30\% to 34\%. Building on this finding, the research explores the use of adapters trained on various programming languages to harness latent information from multilingual datasets. Leveraging the \emph{AdapterFusions}~\cite{pfeiffer2020adapterfusion} architecture, which capitalizes on shared latent information across languages, enhances performance for specific programming language tasks.






The AdapterFusions show promising results. However, both adapters and AdapterFusions are introduced for natural languages. 
Specifically, AdapterFusions still learns more from the language of the target task, not from other programming languages in the dataset, compromising the knowledge it could learn from other programming languages. 
Previous research has shown the advantage of using other languages for a target language, specifically in scenarios of having small datasets~\cite{chen2022transferability, ahmed2021multilingual, wang2023oneAdapter}.
Therefore, we propose \textbf{Adversarial Fusion Adapter (AdvFusion)}, a new architecture that enforces the AdapterFusions to first learn from other programming languages and then from the target programming language. 
We evaluated AdvFusion on code summarization and method name prediction, when applied on CodeBERT and GraphCodeBERT. We experimented with all six programming languages of the CodeSearchNet dataset. In all cases, the results are improved or are on-par with the fully fine-tuned models or when AdapterFusions are used. 
Again, notice that this is achieved by only fine-tuning 0.8\% of the parameters and reducing the training time by a factor of 1.5x.
It is worth mentioning that we chose `Adversarial' for AdvFusion name {as we train the model in an adversarial manner, diverging from the conventional approach of creating adversarial samples.}


Our contributions are as follows. 
\begin{itemize}
    \item Evaluating task-specific adapters for code summarization and method name prediction. 
    \item Investigating the capabilities of AdapterFusions for multi-lingual fine-tuning, in the context of code summarization and method name prediction.
    \item Proposing a new adapter architecture, AdvFusion, for fostering knowledge transfer from other programming languages in the multi-lingual setting. 
\end{itemize}

% \FHF{Write a better significance. This one is just repition of the previosu paragraphs.  }
% \iman{We have already explained the importance of the work in the previous paragraphs. In a nut shell we want to say, 1. PEFT methods have benefits compare to standard finetuning, 2. multilingual fine-tuning works better in software tasks compared to monolingual approach based on \cite{ahmed2021multilingual}, 3. AdapterFusion is proposed to take advantage of PEFT multilingual fine-tuning but it mostly utilize from the language adapter corresponding to its input language 4. we propose advfusion to alleviate this problem, so it is a PEFT multilingual approach that avoids catastrophic forgetting while it can benefit from other languages more than AdapterFution.}

PEFT approaches are attractive choices to tune language models for down stream tasks with less number of parameters both in NLP and SE \cite{pfeiffer2020adapterfusion,pfeiffer2020mad,saberi2023model,wang2023oneAdapter}. The importance of PEFT is more discernible when the computational resources are limited. Additionally, it has been shown that language models do not have good performance for low resource languages \cite{feng2020codebert,guo2020graphcodebert}. Our work sheds light on how we can improve PEFT methods to achieve higher or on-par performance for low-resource languages. 
% We provide results on how multilingual knowledge transfer using AdvFusion can affect the programming languages of CodeXGLUE benchmark. 





The rest of the paper is organized as follows. In Section \ref{section:background}, we provide an overview of necessary background information and then introduce our proposed adapter, AdvFusion, in Section \ref{section:approach}. In Section \ref{section:rq} we provide the research questions and the details of our study, followed by the experimental setup in Section \ref{section:experiments}. Results are explained in Section \ref{section:result} and are further discussed in Section \ref{section:discussion}. Sections \ref{section:related-work} and \ref{section:threat} are dedicated to the related works and threats to validity. Finally, we conclude the paper in Section \ref{section:conclusion}. 



% \FF{the story has a flow now, but we have not talked about the significance of the study and why we should do this!}


% Next, we train an adapter fusion, an attention-based adapter proposed in \cite{pfeiffer2020adapterfusion}, placed on top of a stack of language adapters using a multilingual dataset. It's aim is to select a set of embeddings for a specific task from the language adapters (See Fig. \ref{fig:fusion-internal}). More specifically, when an input is passed through the network, we have embeddings of that input from each language adapter, and the adapter fusion will select a set of embeddings that will maximize the objective function of the downstream task. 
% In NLP, adapter fusions are mainly introduced as a \emph{non-destructive task composition} for transfer learning \cite{pfeiffer2020adapterfusion} where we have a stack of task adapters trained on different downstream tasks, and the adapter fusion will extract a set of embeddings for a particular low-resource language downstream task. 


% However, when trained on a particular target language downstream task, the adapter fusion will tend to activate on the same language adapter more at every layer \cite{pfeiffer2020adapterfusion}. For example, given that the downstream task is for a particular programming language, Ruby, and there are two language adapters trained on two different programming language datasets, Ruby and Java. The adapter fusion sits on top of the language adapters and the adapter fusion will pay more attention to the Ruby language adapter than the Java language adapter. In this case, there will be minimal learning from the Java language adapter.

% Therefore, \textbf{we propose a variant of the adapter fusion, Adversarial Fusion adapter (AdvFusion),  for knowledge extraction from the different programming language adapters and we show that our approach improves the performance of downstream tasks involving low-resource languages and decreases the fine-tuning computational cost for all languages}. AdvFusion enforces the fusion layer to learn more from the other languages for a given target language of a downstream task, instead of focusing on learning from the language adapters, which may cause bias on the language adapter that has the same language as the downstream task. 
% We fine-tune AdvFusion on code summarization in two phases. First, we disable the language adapter that is corresponding to the target language that we expect the model to be fine-tuned on and enforce AdvFusion to learn from the other language adapters on that specific task. For example, for code summarization on Ruby, we disable the Ruby language adapter and train AdvFusion to learn only from the other five language adapters that exist on CodeSearchNet. 
% In the second phase, we enable the muted language adapter (i.e., Ruby language adapter in this example) and fine-tune AdvFusion the second time on \textit{all} the language adapters. 



% \begin{figure}
% \centering
%     \scalebox{.8}{
%     \input{images/Architecture_figure}
%     }
% \caption{Overview of the Transformer architecture with language adapters and AdapterFusion. The pre-trained programming language adapters are placed after the second Add \& Normalization layer inside each Transformer. The output of the language adapters are fed into the AdapterFusion as keys and values; and the output of the feed forward layer is sent to the AdapterFusion as its queries. }
% \label{fig:transformer-arch}
% \end{figure}


\begin{figure}
\centering
    \scalebox{.6}{
    \input{images/internal_fusion}
    }
\caption{Internal structure of AdapterFusion. }

\label{fig:fusion-internal}
\end{figure}


% \begin{figure}
%     \centering
%     \begin{minipage}{0.45\textwidth}
%         \centering
%         \scalebox{.7}{
%         \input{images/Architecture_figure}
%         }
%         \caption{ Overview of the Transformer architecture with language adapters and AdapterFusion. The pre-trained programming language adapters are placed after the second Add \& Normalization layer inside each Transformer. The output of the language adapters are fed into the AdapterFusion as keys and values; and the output of the feed forward layer is sent to the AdapterFusion as its queries. }
%         \label{fig:transformer-arch}
%     \end{minipage}\hfill
%     \begin{minipage}{0.45\textwidth}
%         \centering
%         \scalebox{.7}{
%         \input{images/internal_fusion}
%         }
%         \caption{ Internal structure of AdapterFusion. AdapterFusion is placed on top of a stack of adapters trained on programming languages (i.e., language adapters). The output of the language adapters are fed to the key and value in AdapterFusion and for each query, the AdapterFusion will choose a set of weights from the language adapters.}
%         \label{fig:fusion-internal}
%     \end{minipage}
% \end{figure}





% \textbf{Significance of Study:}
% Adapters are meant to be be used as quick and parameter efficient alternative approach to fully fine tuning the whole models' parameters. We show that it in addition to this, they can improve the performance ..

% In this study, we show that adapter-based monolingual finetuning is not only a quick and parameter-efficient approach, but it can improve the performance of low-resource languages; so it can be used as an \textit{alternative approach to the monolingual finetuning phase on low resource datasets in the future}. Besides, We provide insights into how much each programming language contributes to code summarization for a low-resource language. This contribution is a similarity indicator for different programming languages from the finetuned model's point of view. \iman{Using AdvFusion, researchers could determine which datasets are more useful for a low-resource language and leverage them more than the Fusion adapter in practice.}


==> Sections/Results-old.tex <==

\section{Results} \label{section:result}



% \textcolor{red}{I think you missed explaining the baseline models? or it is not needed? Baseline not backbone.}

% \textcolor{red}{@IMAN: In the results, for all rqs, add what would be compared to what, so the tables and the explanations you mentioned earlier makes sense (multilingual is compared to X, monolingual is compared to Y baseline (include reasons too). }

% \textit{ RQ1: What is the performance of employing adapters in Programming PLMs in terms of training time and model accuracy}
\subsection{ RQ1: Performance of Adapter-Based Fine-tuning}


% \textcolor{red}{1) Think about using the word "task adapter" or just adapter? I think if you say "task" adapter for RQ1 and just adapter or "language" adapter for other RQs, it would bring a lot of questions and confusions. Assess and revise accordingly throughout the paper. We may want to keep it as is for now. Just make sure you mentiuoned the differences AND, WHAT KIND OF ADAPTERS DOES THE ADAPTERFUSION WORK WITH. If ou explain it above, where you introduce adapterfusion, it resolves the issue. }

% \FHF{2) What is the "convetional method" in this paragraph?}
% \iman{it is changed to full fine-tuning}

We assessed the effectiveness of two fine-tuning approaches—using task adapters and the full fine-tuning method—on monolingual datasets. {We incorporated task adapters into both CodeBERT and GraphCodeBERT for the tasks of code summarization and method name prediction}. This allowed us to  assess the performance of task adapters across two baseline models and two target tasks. 


% To evaluate the performance of adapters as an alternative way to finetuning, we trained task adapters on code summarization for each programmin language, separately. 
% The task adapters (CodeBERT+TaskAdapter) are fine-tuned on each language separately. And once, we plugged task adapters to the pretrained model (CodeBERT+TaskAdapter) and only finetuned adapter weights while the pretrained model weights are frozen. We keep the total number of training steps equal for both approaches (i.e., 20000 steps for each one) and use a batch size of 32. 

The obtained BLEU scores and the training times for code summarization are reported in Tables \ref{table:different_methods} and \ref{table:task-adapter-time}, respectively. 
Note that the adapter approach has fewer parameters and lesser training time than the standard way of fine-tuning for all the programming languages. The total number of trainable parameters in standard fine-tuning is $\sim 110$M, while there are $\sim 0.89$M trainable parameters for adapter-based fine-tuning.
The training time (see Table \ref{table:task-adapter-time}) is also reduced by $\sim30\%$ for all languages with adapter-based fine-tuning. Despite having fewer parameters and shorter training times, we observed a performance improvement for most languages and on-par results for the other two.
% The dashed line in Table \ref{table:task-adapter} separates the languages with higher performance improvement from the languages that we got on-par results compare to the baseline. 
% For Ruby, JavaScript, and Go, the improvement of the BLEU scores vary from $7\%$ to $28\%$. For other languages, we have slight improvement or on-par results. 

% , with CodeBERT+TaskAdapter, the BLEU score for Ruby, a low-resource language, has an improvement of $17\%$ on average. Interestingly, for JavaScript and Go, we also observe improvement, where Go has the highest score with 23.21 BELU score. 
% Using CodeBERT+TaskAdapter, we achieve approximately the same results for high-resource languages, as we obtain through the standard approach of fine-tuning on CodeBERT. 



Table \ref{table:different_methods} shows the results of other approaches for code summarization on CodeSearchNet. 
% The dashed line separates the models with multilingual fine-tuning (i.e., \textit{polyglot}GraphCodeBERT and \textit{polyglot}CodeBERT for RQ2) from other models that have monolingual fine-tuning.
As mentioned before, in RQ1, we consider CodeBERT/GraphCodeBERT+TaskAdapter/LoRA with models that are fine-tuned on a single language for a fairer comparison. 
The BLEU scores obtained using CodeBERT/GraphCodeBERT + TaskAdapter are higher or on par with their backbone models. It is important to note that certain baseline models, such as CodeT5, possess approximately 220 million parameters. This parameter count is nearly double that of CodeBERT or GraphCodeBERT. Consequently, making a direct comparison between CodeBERT+TaskAdapters and CodeT5 may not be fair due to this significant difference in parameter size. \iman{We also repeated our experiments using LoRA, a widely-used method in Parameter-Efficient Fine-Tuning (PEFT). The results show that for most programming languages and both baseline models, LoRA's performance is comparable to TaskAdapter's performance.}

{Due to computational restrictions, we used the BLEU scores from the original papers reported for full fine-tuning of CodeBERT and GraphCodeBERT in the context of code summarization. But We ran experiments for code summarization using Task Adapter, LoRA, AdapterFusion, and AdvFusion techniques for both CodeBERT and GraphCodeBERT. However, for method name prediction, we independently conducted and reproduced all experiments.}


We repeat our experiment using the same settings for method name prediction and the results are presented in Table~\ref{table:mnp}. To address the first research question, we compared CodeBERT and GraphCodeBERT that are fine-tuned on each programming language with CodeBERT+TaskAdapter and GraphCodeBERT+TaskAdapter, respectively. The results indicate that task adapter fine-tuning of GraphCodeBERT can result in a decrease in F1-score of up to 4 percent. 
For JavaScript and Go we achieved close results to full fine-tuning of CodeBERT and GraphCodeBERT.
Notably, we employed only $0.89$ million trainable parameters for fine-tuning with task adapter, significantly fewer than the fully fine-tuned model with $110$ million parameters. Training times for method name prediction is shown in Table \ref{table:task-adapter-time-method-name}, 
which shows the training time is reduced by $21\%$ to $25\%$ for all programming languages.

\vspace{3mm}
% \textcolor{red}{Explain more about the method name prediction results. You can explain by saying it is improved/on par for xx languages, etc. The current writing should be expanded.}
 
% \FHF{We don't want to have the SAME table in two of your papers. I am referring to table 4. It is plagiarism. } \iman{some rows are removed, most of them are not repeated.}



\begin{mdframed} [backgroundcolor=gray!20, linewidth=1pt]
\textbf{Insight 2: Adapter-based monolingual fine-tuning of code summarization for high-resource programming languages yields almost the same result with fewer computational resources and less training time than fine-tuning the entire model.}
\end{mdframed}

\vspace{10pt}

\begin{mdframed} [backgroundcolor=gray!20, linewidth=1pt]
\textbf{Insight 3: Adapter-based monolingual fine-tuning of method name prediction yields almost less accuracy with fewer computational resources and less training time than fine-tuning the entire model.}
\end{mdframed}



% \begin{table*}[t!]
% \centering
% \begin{tabular}{l | c | c| c} 
%  \hline
%  Language & \begin{tabular}{@{}c@{}}CodeBERT \\ (\# trainable params: 110M) \end{tabular}   & 
%  \begin{tabular}{@{}c@{}}\textsubscript{+TA} \\ (\# trainable params: 0.89M)  \end{tabular}  & 
%  Improvement \\ [0.5ex] 
%  \hline
%  Ruby & 12.16 & 14.12 & 16\%  \\ 
%  \hdashline
%  JavaScript & 15.67 & 16.80 &7\%   \\ 
%  Go  & 18.07 & 23.21 &  28\% \\ 
% \hdashline
%  Python & 19.06 & 18.47 & -3\% \\ 
%  Java & 17.65 & 18.99 & 7\% \\ 
%  PHP & 25.16 & 25.25 & 0\% \\ 
% \hline
% %    Number of Parameters  & 124M & 21M  \\
% % \hline
% \end{tabular}

% \caption{Performance of task adapters for code summarization on monolingual fine-tuning setting. Note that the dashed line separates Ruby, a low-resource language with the rest, and the second dashed line separates where improvement is achieved when adapters are used. CodeBERT and CodeBERT+TaskAdapter columns indicate the smooth BLEU-4 scores for these models. The last two columns specify the training hours in H:MM format.}
% \label{table:task-adapter}
% \end{table*}

% \textcolor{red}{In table 2, fix the arrows so they are aligned vertically. If you can. This is a nice-to-have feature.}

% \begin{table*}[t!]
%     \centering
%     \begin{tabular}{l | c | c| c} 
%         \hline
%         Language & CodeBERT (110M) & CodeBERT+TaskAdapter (0.89M)  & Improvement \\ [0.5ex] 
%         \hline
%         Ruby & 12.16 & 14.12 & 16\% \textcolor{Gr}{$\uparrow$} \\ 
%         JavaScript & 15.67 & 16.80 &7\%  \textcolor{Gr}{$\uparrow$} \\ 
%         Go  & 18.07 & 23.21 &  28\% \textcolor{Gr}{$\uparrow$} \\ 
%         \hdashline
%         Python & 19.06 & 18.47 & -3\% \textcolor{red}{$\downarrow$} \\ 
%         Java & 17.65 & 18.99 & 7\% \textcolor{Gr}{$\uparrow$} \\ 
%         PHP & 25.16 & 25.25 & 0\% \textcolor{Gr}{$-$}\\ 
%         \hline
%     \end{tabular}

%     \caption{Performance of CodeBERT with task adapters (TA) for code summarization. The results show the monolingual fine-tuning setting. Note that the dashed line separates the languages with smaller datasets from the rest of the programming languages. In all columns the smooth BLEU-4 scores are reported. The last column shows the improvement over the full fine-tuning, when TA are used. The numbers in front of the model names show the number of trainable parameters in millions. }
%     \label{table:task-adapter}
% \end{table*}


% \begin{table*}[t!]
% \centering
% \begin{tabular}{l | c| c} 
%  \hline
%  Language & \begin{tabular}{@{}c@{}c@{}}CodeBERT \\
%  Training Time \\ 
%  (20,000 steps)  \end{tabular}   & 
%  \begin{tabular}{@{}c@{}c@{}} CodeBERT+TaskAdapter  \\ Training Time \\ (20,000 steps)  \end{tabular}  \\ [0.5ex] 
%  \hline
%  Ruby &  8:12 & ~5:28 \\ 
%  JavaScript &  8:13 & ~5:44  \\ 
%  Go  &   8:31 & ~5:36\\ 
%  Python  & 8.13 & ~5:23\\ 
%  Java &  8:14 & ~5:41\\ 
%  PHP &  8:26 & ~5:38\\ 
% \hline
% %    Number of Parameters  & 124M & 21M  \\
% % \hline
% \end{tabular}

% \caption{Time efficiency of task adapters for code summarization on monolingual fine-tuning setting. The numbers specify the training time in minutes, and the last column shows the improvement percentage (i.e., how much the training time is reduced.}
% \label{table:task-adapter}
% \end{table*}



\begin{table}
    \centering
    \scalebox{.95}{
    \begin{tabular}{c|c|c|c}
    \hline
         Language & CodeBERT & CodeBERT+TaskAdapter & Time reduction\\
         \hline
         Ruby &  492 & 328 & -33\% \textcolor{Gr}{$\downarrow$}\\ 
         JavaScript &  493 & 344 & -30\% \textcolor{Gr}{$\downarrow$}\\ 
         Go  &   511 & 336 & -34\% \textcolor{Gr}{$\downarrow$}\\ 
         Python  & 493 & 323 & -34\% \textcolor{Gr}{$\downarrow$}\\ 
         Java &  494 & 341 & -31\% \textcolor{Gr}{$\downarrow$}\\ 
         PHP &  506 & 338 & -33\% \textcolor{Gr}{$\downarrow$}\\
         \hline
    \end{tabular}
    }
    \caption{Task adapter time efficiency for code summarization in monolingual fine-tuning. Numbers represent training time in minutes, with the last column showing percentage improvement. Times reflect training for 20,000 steps.}
    \label{table:task-adapter-time}
\end{table}


\begin{table}
    \centering
    \scalebox{.95}{
    \begin{tabular}{c|c|c|c}
    \hline
         Language & CodeBERT & CodeBERT+TaskAdapter & Time reduction\\
         \hline
         Ruby &  105 & 80 & -24\% \textcolor{Gr}{$\downarrow$}\\ 
         JavaScript &  110 & 84 & -23\% \textcolor{Gr}{$\downarrow$}\\ 
         Go  &   104 & 82 & -21\% \textcolor{Gr}{$\downarrow$}\\ 
         Python  & 106 & 79 & -25\% \textcolor{Gr}{$\downarrow$}\\ 
         Java &  105 & 83 & -21\% \textcolor{Gr}{$\downarrow$}\\ 
         PHP &  104 & 81 & -22\% \textcolor{Gr}{$\downarrow$}\\
         \hline
    \end{tabular}
    }
    \caption{Task adapters for method name prediction in monolingual fine-tuning: training time (minutes) for 5,000 steps and improvement percentage. }
    \label{table:task-adapter-time-method-name}
\end{table}





\begin{table*}[t!]
\centering

\begin{tabular}{|l | c | c| c| c| c| c|} 
 \hline
 Models & Ruby & JavaScript & Go & Python & Java & PHP \\ [0.5ex] 
  \hline
 GraphCodeBERT+AdvFusion & 16.47 & 15.89  & 19.96  & 18.49 & 18.97  & 24.83  \\ 
   % CodeBERT + TypeAdapter & 16.20 & 16.12 &\textbf{24.45} & 18.31 & 19.88 & 25.49 \\ 
 GraphCodeBERT+AdapterFusion & 15.57 & 14.49  & 18.21 & 17.86  & 18.31  & 23.54 \\ 

 GraphCodeBERT+TaskAdapter & 14.39 & 14.53  & 18.47 & 17.88  & 17.29  & 23.36 \\ 

 GraphCodeBERT+LoRA & 14.48 & 14.63  & 17.8 & 18.49  & 17.16  & 24.13 \\ 
% \hline
%    GraphCodeBERT + TaskAdapter & 13.81 & JS &Go & python & java & php
%    \\
 % \hline
 \hdashline
 CodeBERT+AdvFusion & \textbf{16.53} & \textbf{16.80} & \textbf{24.09} & 18.28 & 19.94 &25.20  \\ 
   % CodeBERT + TypeAdapter & 16.20 & 16.12 &\textbf{24.45} & 18.31 & 19.88 & 25.49 \\ 
 CodeBERT+AdapterFusion & 15.77 & 16.22 & 24.01 & 18.40 & 19.85 & 25.17 \\ 

 CodeBERT+TaskAdapter & 14.12 & 15.67 &22.21 & 18.47 & 18.99 & 25.55 \\ 

 CodeBERT+LoRA & 12.27 & 13.67  &19.01 & 17.07 & 16.58 & 23.08 \\ 
% \hline
%    GraphCodeBERT + TaskAdapter & 13.81 & JS &Go & python & java & php
%    \\
\hline
 
 $polyglot$GraphCodeBERT \cite{ahmed2021multilingual} & 14.95 & 15.79 &18.92 & 18.90 & 19.91 & 26.15  \\ 
 $polyglot$CodeBERT \cite{ahmed2021multilingual} & 14.75 & 15.80 &18.77 & 18.71 & 20.11 & \textbf{26.23} \\ 
 \hdashline
 CodeT5 \cite{wang2021codet5} & 15.69 & 16.24 &19.76 & \textbf{20.36} & \textbf{20.46} & 26.09 \\ 
 % ProphetNet-Code \cite{qi2021prophetnet} & 14.37 & 16.60  &18.43 & 17.87 & 19.39 & 24.57\\ 
 % PLBART \cite{ahmad2021unified} & 14.11 & 15.56 &18.91 & 19.30 & 18.45 & 23.58 \\ 
 GraphCodeBERT   & 12.62 & 14.79 &18.40 & 18.02 & 19.22 & 25.45\\ 
 CodeBERT  & 12.16 & 14.90 &18.07 & 19.06 & 17.65 & 25.16 \\ 
 RoBERTa \cite{zhuang2021robustly}  & 11.17 & 11.90 &17.72 & 18.14 & 16.47 & 24.02 \\ 
 % Transformer \cite{vaswani2017attention} & 11.18 & 11.59 &16.38 & 15.81 & 16.26 & 22.12\\ 
 % seq2seq \cite{sutskever2014sequence}  & 9.64 & 10.21 &13.98 & 15.93 & 15.09 & 21.08\\ 
 \hline
\end{tabular}




\caption{Smooth BLEU-4 scores on code summarization.
%CodeBERT\textsubscript{Fusion} is fine-tuned on multiple languages, so we should compare it with $polyglot$CodeBERT, same as for \textit{AdvFusion}CodeBERT. 
}
\label{table:different_methods}
\end{table*}




\begin{table*}[!t]
\centering
\begin{adjustbox}{width=0.9\textwidth,center}
\begin{tabular}{@{}cccccccccccccccccccccccc@{}}
\toprule
Model &\multicolumn{3}{c}{Ruby}  &  & \multicolumn{3}{c}{Javascript} &  & \multicolumn{3}{c}{Go} &  & \multicolumn{3}{c}{Python} &  & \multicolumn{3}{c}{Java} &  & \multicolumn{3}{c}{php}\\ \cline{2-4}\cline{6-8} \cline{10-12}\cline{14-16} \cline{18-20} \cline{22-24} \\[-1em]
&  $P$  & $R$ & $F1$ &  & $P$ & $R$ & $F1$ &  & $P$ & $R$ & $F1$ &  & $P$ & $R$ & $F1$ &  & $P$ & $R$ & $F1$ &  & $P$ & $R$ & $F1$  \\ [1em] 
 CodeBERT &  0.37   &   0.32    &   0.33    &  &   0.19    &   0.16  &   0.17    
& &  0.46   &   0.42  &  0.43   &  &   0.49  &  0.45  &  0.45  & &  0.45   & 0.40   &  0.41   & &  0.49  &  0.44  &  0.45 \\ [1em] 

\specialcell{CodeBERT + \\TaskAdapter} &  0.35   &   0.30    &   0.30    &  &   0.19    &   0.14  &   0.16    
& &  0.45   &   0.40  &  0.41   &  &   0.44  &  0.34  &  0.37  & &  0.43   & 0.34   &  0.37   & &  0.45  &  0.38  &  0.40 \\ [1em]

\specialcell{CodeBERT + \\AdapterFusion} &  0.38   &   0.30    &   0.32    &  &   0.19    &   0.14  &   0.16    
& &  0.45   &   0.40  &  0.41   &  &   0.44  &  0.34  &  0.37  & &  0.43   & 0.34   &  0.37   & &  0.45  &  0.38  &  0.40 \\ [1em]

\specialcell{CodeBERT + \\AdvFusion} &  0.38   &   0.32    &   0.34    &  &   0.19    &   0.14  &   0.16    
& &  0.45   &   0.40  &  0.41   &  &   0.44  &  0.34  &  0.37  & &  0.43   & 0.34   &  0.37   & &  0.45  &  0.38  &  0.40 \\ [1em]

%  \specialcell{Polyglot\\CodeBERT} &  \textbf{0.53}   &   \textbf{0.49}    &   \textbf{0.49}    &  &   0.45    &   0.40  &   0.41    
% & &  0.56   &   0.53  &  0.52   &  &   \textbf{0.50}  &  \textbf{0.45}  &  \textbf{0.46}  & &  0.56   & 0.52   &  0.52   & &  0.57  &  0.53  &  0.53 \\ [1em]
 \specialcell{Graph\\CodeBERT} &  0.40   &   0.36    &   0.37    &  &   0.27    &   0.23  &   0.24    
& &  0.48   &   0.44  &  0.45   &  &   0.49  &  0.43  & 0.44  & &  0.47   & 0.41   &  0.43  & &  0.50  &  0.45  &  0.46 \\[1em]

 \specialcell{Graph\\CodeBERT + \\TaskAdapter} &  0.40   &   0.33    &   0.35    &  &   0.24    &   0.22  &   0.23    
& &  0.47   &   0.42  &  0.43   &  &   0.47  &  0.38  & 0.40  & &  0.45   &  0.37   &  0.40   & &  0.48  &  0.41  &  0.43 \\[1em]

 \textbf{\specialcell{ Graph\\CodeBERT + \\AdapterFusion}} &  0.40   &   0.30    &   0.35    &  &   0.57    &   0.57  &   0.57   
& &  0.95   &   0.94  &  0.94   &  &   0.48  &  0.38  & 0.41  & &  0.85   &  0.85   &  0.85   & &  0.81  &  0.80  &  0.80 \\[1em]

 \textbf{\specialcell{ Graph\\CodeBERT + \\AdvFusion}} &  0.42   &   0.32    &   0.36    &  &   \textbf{0.58}    &   \textbf{0.58}  &   \textbf{0.58}   
& &  \textbf{0.96}   &   \textbf{0.96}  &  \textbf{0.96}   &  &   0.49  &  0.40  & 0.42  & &  \textbf{0.85}   &  \textbf{0.85}   &  \textbf{0.85}   & &  \textbf{0.83}  &  \textbf{0.80}  &  \textbf{0.81} \\[1em]

 \bottomrule
\end{tabular}
\end{adjustbox}
\caption{
The Precision (P), Recall (R), and F1-Score (F1) metrics were assessed on each programming language across various settings.}
\label{table:mnp}
\end{table*}



\subsection{RQ2: Performance of Multilingual Fine-Tuning with AdvFusion}

% \FHF{1) I did not read 6.2, the RQ2 results. Please first revise RQ2 and its explanation in section 4.1, and its methodology in 4.2. Then revise 6.2. Make sure you read the introduction first! }

% \FHF{2) We discussed the training time of Advfusion and AdapterFusions, and that Advfusion is using the same number of steps (?) of AdapterFusions. So the training times are the same. Add this discussion somewhere in the results, when you are discussing them.}

% \FF{Make sure you have the training time and its discussion for both RQs.}

In this RQ, we evaluate how much improvement we could gain by using other programming languages, therefore, transferring knowledge in the multilingual fine-tuning of code-LMs. 
In this RQ, we aggregate knowledge in two settings: AdapterFusion and AdvFusion, as explained below.

\subsubsection{AdapterFusion}


Here, we gauge the effectiveness of code summarization using AdapterFusions. Specifically, we evaluate the performance of CodeBERT+Fusion and GraphCodeBERT+Fusion models on code summarization. Additionally, we measure the accuracy of method name prediction using the CodeBERT+Fusion and GraphCodeBERT+Fusion models. 

% \textcolor{red}{Add fusion results.}
As shown in Table \ref{table:different_methods}, CodeBERT+Fusion and GraphCodeBERT+Fusion outperforms the \textit{polyglot} models, which indicates that by multilingual fine-tuning  AdapterFusion, we can achieve better results than multilingual fine-tuning the entire weights of CodeBERT.

In Table \ref{table:multilingual-improvement}, we show the BLEU scores for multilingual CodeBERT (i.e., \textit{polyglot}CodeBERT) \cite{ahmed2021multilingual} and 
CodeBERT + AdvFusion. 
Note that both approaches are using the same code-LMs, but the fine-tuning strategy is different. \textit{polyglot}CodeBERT is fine-tuned on the entire model weights, while CodeBERT + AdvFusion is only fine-tuned on the weights of AdvFusion and the language adapters. 
With CodeBERT + AdvFusion, we achieve $12\%$ improvement for Ruby. 
In this setting, we also observe that JavaScript and Go are improved by 6\% and 28\%, respectively.
This could be related to their large amount of training data (see bimodal statistics in Table \ref{table:plm}). Though they have 3 to 6 times more training data than Ruby, they still have much fewer samples as compared to the other three languages, Python, Java, and PHP. Therefore, they still can learn from the other higher resource languages. 
The results for the other languages, Python, Java, and PHP, are on par with \textit{polyglot}CodeBERT.


The performance of GraphCodeBERT+AdapterFusion in the method name prediction task is presented in Table \ref{table:mnp}. The results show huge improvement of 152\%, 123\%, 112\%, and 88\% for Javascript, Go, Java, and PHP, respectively, when compared to the monolingual adapter-based approach. It's worth noting that for Ruby and Python, the observed changes were not statistically significant.

% We compared our approach with Multilingual CodeBERT \cite{ahmed2021multilingual} model as a baseline which is finetuned on CodeSearchNet \cite{husain2019codesearchnet}. 
\subsubsection{AdvFusion}

We then repeat the previous experiments by replacing AdapterFusion with AdvFusion. We evaluate the effectiveness of AdvFusion in two contexts: code summarization and method name prediction using CodeBERT and GraphCodeBERT, with AdvFusion integrated into the code-LMs.

Note that \textit{AdvFusion} is trained in two phases, the first phase is performed once for all languages (Step 1 of the AdvFusion, see Section \ref{phase1}), and the second phase is conducted on each language (Step 2 of the AdvFusion, see Section \ref{phase2}).
%As an intuitive explanation for alleviating knowledge interference, \textit{AdvFusion}CodeBERT will not be allowed to change the general representations we have learned for each language (in language adapters). Consequently, low-resource language representations will not be affected by high-resource datasets.


In terms of parameter efficiency, CodeBERT + AdvFusion is more efficent than \textit{polyglot}CodeBERT. \textit{polyglot}CodeBERT has 110M trainable parameters, while the total number of trainable parameters in CodeBERT + AdvFusion is about 21M (a 80\% reduction). 
% Note that total number of trainable parameters when we only use task adapters is 0.89M, while it is 21M when we plug adapter fusion or AdvFusion to the model. This is due to the fact that language and task adapters have a simple feed-forward architecture, while AdvFusion and adapter fusion have attention mechanism.
% \textcolor{red}{Explain why there are 21M compared to task adapters with only 0.89M.}

{In terms of training time, as shown in Table \ref{table:multilingual-improvement}, the average fine-tuning time for the entire weights of CodeBERT took $\sim 8$ hours. On the other hand, the first phase in CodeBERT + AdvFusion is performed once and took 3:25 hours while the second phase is done separately for each programming language, and the average fine-tuning time for all languages is 4:27 hours in CodeBERT + AdvFusion, a reduction of $ \sim44 \%$ as compared to the training time using the entire weights of CodeBERT.}


\vspace{10pt}
\begin{mdframed} [backgroundcolor=gray!20, linewidth=1pt]
\textbf{Insight 4: \textit{AdvFusion} improve the performance for low-resource languages while having on par results for high-resource languages with lesser training time and fewer trainable parameters.}
\end{mdframed}



\begin{table}[t!]
\centering
\begin{tabular}{l | c | c| c} 
 \hline
 Language & \begin{tabular}{@{}c@{}}\textit{polyglot} \\ CodeBERT\end{tabular}   & 
 \begin{tabular}{@{}c@{}} CodeBERT + \\ AdvFusion \end{tabular}   & 
 Improvement  \\ [0.5ex] 
 \hline
 Ruby & 14.75 & 16.53 & 12\%   \\ 
   Javascript & 15.80 & 16.80 &6\%   \\ 
 Go  & 18.77 & 24.09 &  28\%  \\ 
\hdashline
 Python & 18.71 & 18.28 & 0\% \\ 
 Java & 20.11 & 19.94 & 0\% \\ 
 PHP & 26.23 & 25.20 & 0\% \\ 
\hline
%    Number of Parameters  & 124M & 21M  \\
% \hline
\end{tabular}

\caption{Effectiveness of using AdvFusion for code summarization in the multilingual fine-tuning setting. The first dashed line separates the results where improvement is observed. The first two columns indicate the smooth BLEU-4 score for each language.
}
\label{table:multilingual-improvement}
\end{table}


\begin{table}[t!]
\centering
\begin{tabular}{l | c| c| c} 
 \hline
 Language &  \begin{tabular}{@{}c@{}}\textit{polyglot}\\ CodeBERT  \end{tabular}   & 
 \begin{tabular}{@{}c@{}c@{}}  CodeBERT + \\ \textit{AdvFusion} \end{tabular}  & Time reduction \\ [0.5ex]  
 \hline
 Ruby &  8:06 & 4:09  & -48\% \textcolor{Gr}{$\downarrow$}  \\ 
 \hdashline
   Javascript &  8:05 &  4:22  & -45\% \textcolor{Gr}{$\downarrow$} \\ 
 Go  &  8:07 & 4:50& -40\% \textcolor{Gr}{$\downarrow$}\\ 
\hdashline
 Python  & 8.03 & 5:09 & -36\% \textcolor{Gr}{$\downarrow$}\\ 
 Java & 8:04 & 4:27 & -44\% \textcolor{Gr}{$\downarrow$}\\ 
 PHP  & 8:06 & 4:47 & -41\% \textcolor{Gr}{$\downarrow$}\\ 
\hline
%    Number of Parameters  & 124M & 21M  \\
% \hline
\end{tabular}

\caption{Effectiveness of using AdvFusion for code summarization in the multilingual fine-tuning setting.
 The columns specify the training hours in H:MM format. 
}
\label{table:multilingual-improvement}
\end{table}



\subsection{RQ3: Languages' Contribution for a Low-Resource Programming Language}
% \FHF{see my other note on using the words "task" and "language" before adapter, and revise if needed.}\\
Here, we evaluate the contribution of each language (from the language adapters) on Ruby for code summarization when using AdvFusion as compared to AdapterFusions.
We extract the attention at AdvFusion and AdapterFusion when we fine-tune  CodeBERT + AdvFusion and CodeBERT+Fusion, respectively (separate experiments). 
% The goal is to evaluate other languages' contribution in both finetuned models by attention analysis. We fed the Ruby dataset to both models and grabbed the attention we got from both models. 
% Specifically, we first aggregate the attention we gain from all the tokens of each language at each (fusion or Adversarial fusion) layer. Then, we normalizedthe attentions using min-max approach at each layer to calculate the percentage of each language participation. 
Fig.~\ref{fig:fusion-ruby} demonstrates the contribution of each language at each layer in CodeBERT+Fusion when the Ruby test dataset is fed to the fine-tuned model. 
The x-axis shows the attention score and the y-axis shows the contribution of each language at each layer in percentage. The color bars show the contributions from each of the six programming languages. In most layers, a high percentage of attention (more than 80\%) is towards Ruby (the gray bar). This shows that AdapterFusion tends to pay more attention to the language adapter that corresponds to the same language of the input. In other words, not much is learned from other programming languages.
% which has been mentioned in adapter fusion paper \cite{pfeiffer2020adapterfusion}. 

Fig.~\ref{fig:adv-fusion-ruby} shows the contribution of each language in CodeBERT + AdvFusion when the Ruby test dataset is fed to the fine-tuned model. The y-axis is the layer number in CodeBERT, and the x-axis shows the percentage of contribution of each language. Here, AdvFusion pays more attention to other programming languages as shown in Fig.~\ref{fig:fusion-ruby}. For instance, Ruby has the following learning: it learns more from Go in the second layer (i.e., $52.9\%$ of attention are grabbed from Go adapter), it learns more from Python than Ruby in the forth layer (i.e., $56.2\%$), and it learns more from JavaScript in layer seven. Even in the higher layers, learning from other languages is continued and the attention is distributed to other languages, and not only focused on Ruby. 
More interestingly, PHP is the most resourceful language in the dataset, but its contribution for Ruby is less than other languages. This suggests that there is no relationship between the size of the language dataset and its contribution to Ruby.

\vspace{3mm}

\begin{mdframed} [backgroundcolor=gray!20, linewidth=1pt]
\textbf{Insight 5: Low resource language, Ruby, could benefit from the other resourceful languages differently in different layers.}
\end{mdframed}

\vspace{10pt} 

\begin{mdframed} [backgroundcolor=gray!20, linewidth=1pt]
\textbf{Insight 6: Higher resource languages do not necessarily contribute more to the low-resource language, Ruby.}
\end{mdframed}

% \textcolor{red}{ADD DETAILS. SEE MY COMMENTS.}






\begin{figure}

\includegraphics[width=\columnwidth]{images/adv-ruby.png}
\centering
\caption{The attention contribution from each programming language at each layer when we feed the Ruby test dataset to the fine-tuned AdvFusion model.}
\label{fig:adv-fusion-ruby}
\end{figure}





% \begin{table*}[t!]
% \centering
% \begin{tabular}{|l | c | c| c| c| c| c|} 
%  \hline
%  Models & Ruby & JavaScript & Go & Python & Java & PHP \\ [0.5ex] 
%   \hline
%  $AdvFusion$GraphCodeBERT & 16.37 & 15.89  & 19.96  & 18.49 & 18.97  & 24.83  \\ 
%    % CodeBERT + TypeAdapter & 16.20 & 16.12 &\textbf{24.45} & 18.31 & 19.88 & 25.49 \\ 
%  GraphCodeBERT+Fusion & 15.57 & 14.49  & 18.21 & 17.86  & 18.31  & 23.54 \\ 

% % \hline
% %    GraphCodeBERT + TaskAdapter & 13.81 & JS &Go & python & java & php
% %    \\
%  \hline
%  $AdvFusion$CodeBERT & \textbf{16.53} & \textbf{16.80} & \textbf{24.09} & 18.28 & 19.94 &25.20  \\ 
%    % CodeBERT + TypeAdapter & 16.20 & 16.12 &\textbf{24.45} & 18.31 & 19.88 & 25.49 \\ 
%  CodeBERT+Fusion & 15.77 & 16.22 & 24.01 & 18.40 & 19.85 & 25.17 \\ 

%  CodeBERT+TaskAdapter & 14.12 & 15.67 &23.21 & 18.47 & 18.99 & 25.55 \\ 
% % \hline
% %    GraphCodeBERT + TaskAdapter & 13.81 & JS &Go & python & java & php
% %    \\
% \hline
 
%  $polyglot$GraphCodeBERT \cite{ahmed2021multilingual} & 14.95 & 15.79 &18.92 & 18.90 & 19.91 & 26.15  \\ 
%  $polyglot$CodeBERT \cite{ahmed2021multilingual} & 14.75 & 15.80 &18.77 & 18.71 & 20.11 & \textbf{26.23} \\ 
%  \hdashline
%  CodeT5 \cite{wang2021codet5} & 15.69 & 16.24 &19.76 & \textbf{20.36} & \textbf{20.46} & 26.09 \\ 
%  ProphetNet-Code \cite{qi2021prophetnet} & 14.37 & 16.60  &18.43 & 17.87 & 19.39 & 24.57\\ 
%  PLBART \cite{ahmad2021unified} & 14.11 & 15.56 &18.91 & 19.30 & 18.45 & 23.58 \\ 
%  GraphCodeBERT   & 12.62 & 14.79 &18.40 & 18.02 & 19.22 & 25.45\\ 
%  CodeBERT  & 12.16 & 14.90 &18.07 & 19.06 & 17.65 & 25.16 \\ 
%  RoBERTa \cite{zhuang2021robustly}  & 11.17 & 11.90 &17.72 & 18.14 & 16.47 & 24.02 \\ 
%  Transformer \cite{vaswani2017attention} & 11.18 & 11.59 &16.38 & 15.81 & 16.26 & 22.12\\ 
%  seq2seq \cite{sutskever2014sequence}  & 9.64 & 10.21 &13.98 & 15.93 & 15.09 & 21.08\\ 
%  \hline
% \end{tabular}




% \caption{Smooth BLEU-4 scores on code summarization.  CodeBERT+TaskAdapter is fine-tuned on the monolingual datasets (same as CodeBERT). If we encourage the model weights to be closer to the pre-trained model, we could improve the fine-tuning task without additional data. %CodeBERT\textsubscript{Fusion} is fine-tuned on multiple languages, so we should compare it with $polyglot$CodeBERT, same as for \textit{AdvFusion}CodeBERT. 
% }
% \label{table:different_methods}
% \end{table*}




==> images/Architecture_figure.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[rounded corners, x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,584); %set diagram left start at 0, and has height of 584

%Rounded Rect [id:dp4508323193467638] 
\draw  [fill={rgb, 255:red, 248; green, 247; blue, 255 }  ,fill opacity=1 ][line width=1.5]  (190,59.77) .. controls (190,39.19) and (206.69,22.5) .. (227.27,22.5) -- (446.73,22.5) .. controls (467.31,22.5) and (484,39.19) .. (484,59.77) -- (484,483.23) .. controls (484,503.81) and (467.31,520.5) .. (446.73,520.5) -- (227.27,520.5) .. controls (206.69,520.5) and (190,503.81) .. (190,483.23) -- cycle ;
%Straight Lines [id:da33185925799900695] 
\draw [color={rgb, 255:red, 38; green, 19; blue, 19 }  ,draw opacity=1 ][line width=1.5]    (340,536.5) -- (340,487) ;
\draw [shift={(340,483)}, rotate = 90] [fill={rgb, 255:red, 38; green, 19; blue, 19 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Curve Lines [id:da15112378632237533] 
\draw [color={rgb, 255:red, 38; green, 19; blue, 19 }  ,draw opacity=1 ][line width=1.5]    (317.06,486.27) .. controls (317.63,504.51) and (322.33,514.18) .. (340,513.25) .. controls (357.86,512.31) and (360.7,505.85) .. (360.98,486.8) ;
\draw [shift={(361,483)}, rotate = 90] [fill={rgb, 255:red, 38; green, 19; blue, 19 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
\draw [shift={(317,482)}, rotate = 90] [fill={rgb, 255:red, 38; green, 19; blue, 19 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da827355102305328] 
\draw [color={rgb, 255:red, 38; green, 19; blue, 19 }  ,draw opacity=1 ][line width=2.25]    (339,428.5) -- (339,457) ;
%Straight Lines [id:da9658267846213033] 
\draw [color={rgb, 255:red, 38; green, 19; blue, 19 }  ,draw opacity=1 ][line width=2.25]    (339,366.5) -- (339,395.5) ;
%Straight Lines [id:da10402210926959543] 
\draw [color={rgb, 255:red, 38; green, 19; blue, 19 }  ,draw opacity=1 ][line width=2.25]    (339,310.5) -- (339,344) ;
%Straight Lines [id:da2888412524874291] 
\draw [color={rgb, 255:red, 38; green, 19; blue, 19 }  ,draw opacity=1 ][line width=1.5]    (341,385.5) -- (204,385.5) -- (204,298.5) -- (268,298.5) ;
\draw [shift={(272,298.5)}, rotate = 180] [fill={rgb, 255:red, 38; green, 19; blue, 19 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da31229286569755144] 
\draw [color={rgb, 255:red, 38; green, 19; blue, 19 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=0.61 ][line width=1.5]    (340,163.5) -- (340,191.5) ;
\draw [shift={(340,159.5)}, rotate = 90] [fill={rgb, 255:red, 38; green, 19; blue, 19 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da4445467914930803] 
\draw [color={rgb, 255:red, 38; green, 19; blue, 19 }  ,draw opacity=1 ][line width=1.5]    (350,163.5) -- (350,192.5) ;
\draw [shift={(350,159.5)}, rotate = 90] [fill={rgb, 255:red, 38; green, 19; blue, 19 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da9841294017683555] 
\draw [color={rgb, 255:red, 38; green, 19; blue, 19 }  ,draw opacity=1 ][line width=1.5]    (360,163.5) -- (360,191.5) ;
\draw [shift={(360,159.5)}, rotate = 90] [fill={rgb, 255:red, 38; green, 19; blue, 19 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da7763680856457562] 
\draw [color={rgb, 255:red, 38; green, 19; blue, 19 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=0.61 ][line width=1.5]    (263,163.5) -- (263,191.5) ;
\draw [shift={(263,159.5)}, rotate = 90] [fill={rgb, 255:red, 38; green, 19; blue, 19 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da8967344268089401] 
\draw [color={rgb, 255:red, 38; green, 19; blue, 19 }  ,draw opacity=1 ][line width=1.5]    (273,163.5) -- (273,192.5) ;
\draw [shift={(273,159.5)}, rotate = 90] [fill={rgb, 255:red, 38; green, 19; blue, 19 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da8524322479070345] 
\draw [color={rgb, 255:red, 38; green, 19; blue, 19 }  ,draw opacity=1 ][line width=1.5]    (283,163.5) -- (283,191.5) ;
\draw [shift={(283,159.5)}, rotate = 90] [fill={rgb, 255:red, 38; green, 19; blue, 19 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da21642424997917353] 
\draw [color={rgb, 255:red, 38; green, 19; blue, 19 }  ,draw opacity=1 ][line width=1.5]    (340,327.5) -- (433,328.5) -- (433,162.5) ;
\draw [shift={(433,158.5)}, rotate = 90] [fill={rgb, 255:red, 38; green, 19; blue, 19 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da5590738168584097] 
\draw [color={rgb, 255:red, 38; green, 19; blue, 19 }  ,draw opacity=1 ][line width=1.5]    (340,327.5) -- (214,326.5) -- (214,235.5) -- (237,235.5) ;
\draw [shift={(241,235.5)}, rotate = 180] [fill={rgb, 255:red, 38; green, 19; blue, 19 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da8518206573923552] 
\draw [color={rgb, 255:red, 38; green, 19; blue, 19 }  ,draw opacity=1 ][line width=1.5]    (340,327.5) -- (214,326.5) -- (214,224.5) -- (243,224.5) ;
\draw [shift={(247,224.5)}, rotate = 180] [fill={rgb, 255:red, 38; green, 19; blue, 19 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da14092877527551617] 
\draw [color={rgb, 255:red, 38; green, 19; blue, 19 }  ,draw opacity=1 ][line width=2.25]    (344,90.5) -- (344,108.5) ;
%Straight Lines [id:da27640448701486786] 
\draw [color={rgb, 255:red, 38; green, 19; blue, 19 }  ,draw opacity=1 ][line width=1.5]    (340.5,385.5) -- (203.5,385.5) -- (203.5,71.5) -- (268,71.5) ;
\draw [shift={(272,71.5)}, rotate = 180] [fill={rgb, 255:red, 38; green, 19; blue, 19 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da04907442828060504] 
\draw [color={rgb, 255:red, 38; green, 19; blue, 19 }  ,draw opacity=1 ][line width=2.25]    (344,10.5) -- (344,57.5) ;
\draw [shift={(344,5.5)}, rotate = 90] [fill={rgb, 255:red, 38; green, 19; blue, 19 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;
%Shape: Rectangle [id:dp5419208013788495] 
\draw  [fill={rgb, 255:red, 128; green, 147; blue, 241 }  ,fill opacity=1 ][line width=1.5]  (239,205.25) -- (414,205.25) -- (414,257.25) -- (239,257.25) -- cycle ;
%Shape: Rectangle [id:dp07515895347510937] 
\draw  [fill={rgb, 255:red, 128; green, 147; blue, 241 }  ,fill opacity=1 ][line width=1.5]  (247,196.25) -- (422,196.25) -- (422,248.25) -- (247,248.25) -- cycle ;
%Straight Lines [id:da08280798923342192] 
\draw [color={rgb, 255:red, 38; green, 19; blue, 19 }  ,draw opacity=1 ][line width=1.5]    (346.09,240.5) -- (347,283.5) ;
\draw [shift={(346,236.5)}, rotate = 88.78] [fill={rgb, 255:red, 38; green, 19; blue, 19 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da039096439051388154] 
\draw [color={rgb, 255:red, 38; green, 19; blue, 19 }  ,draw opacity=1 ][line width=1.5]    (338,249.5) -- (338,282.5) ;
\draw [shift={(338,245.5)}, rotate = 90] [fill={rgb, 255:red, 38; green, 19; blue, 19 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da8927315564167555] 
\draw [color={rgb, 255:red, 38; green, 19; blue, 19 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=0.61 ][line width=1.5]    (331,259.5) -- (331,283.5) ;
\draw [shift={(331,255.5)}, rotate = 90] [fill={rgb, 255:red, 38; green, 19; blue, 19 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da04159444380938582] 
\draw [color={rgb, 255:red, 38; green, 19; blue, 19 }  ,draw opacity=1 ][line width=1.5]    (340,327.5) -- (214,326.5) -- (214,213.5) -- (252,213.5) ;
\draw [shift={(256,213.5)}, rotate = 180] [fill={rgb, 255:red, 38; green, 19; blue, 19 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;

% Text Node
\draw  [fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ][line width=1.5]   (253.5,451.5) -- (428.5,451.5) -- (428.5,484.5) -- (253.5,484.5) -- cycle  ;
\draw (341,468) node   [align=left] {\begin{minipage}[lt]{116.28pt}\setlength\topsep{0pt}
\begin{center}
{\small \textbf{Multi-Head Attention}}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 202; green, 207; blue, 133 }  ,fill opacity=1 ][line width=1.5]   (270,396.25) -- (417,396.25) -- (417,429.25) -- (270,429.25) -- cycle  ;
\draw (343.5,412.75) node   [align=left] {\begin{minipage}[lt]{97.24pt}\setlength\topsep{0pt}
\begin{center}
\textbf{{\small Add \& Norm}}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 77; green, 179; blue, 252 }  ,fill opacity=1 ][line width=1.5]   (253,339.75) -- (428,339.75) -- (428,372.75) -- (253,372.75) -- cycle  ;
\draw (340.5,356.25) node   [align=left] {\begin{minipage}[lt]{116.28pt}\setlength\topsep{0pt}
\begin{center}
\textbf{{\small Feed Forward }}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 128; green, 147; blue, 241 }  ,fill opacity=1 ][line width=1.5]   (254,187.25) -- (429,187.25) -- (429,239.25) -- (254,239.25) -- cycle  ;
\draw (341.5,213.25) node   [align=left] {\begin{minipage}[lt]{116.28pt}\setlength\topsep{0pt}
\begin{center}
\textbf{{\small Programming Language Adapters}}
\end{center}

\end{minipage}};
% Text Node
\draw  [color={rgb, 255:red, 38; green, 19; blue, 19 }  ,draw opacity=1 ][fill={rgb, 255:red, 154; green, 189; blue, 151 }  ,fill opacity=1 ][line width=1.5]   (213,109.5) -- (464,109.5) -- (464,161.5) -- (213,161.5) -- cycle  ;
\draw (345.5,130.5) node   [align=left] {\begin{minipage}[lt]{167.96pt}\setlength\topsep{0pt}
\begin{center}
\textbf{{\small {\fontfamily{helvet}\selectfont AdapterFusion}}}
\end{center}

\end{minipage}};
% Text Node
\draw (272.5,148.25) node   [align=left] {\begin{minipage}[lt]{26.52pt}\setlength\topsep{0pt}
\begin{center}
\textbf{{\footnotesize Key}}
\end{center}

\end{minipage}};
% Text Node
\draw (350.5,148.25) node   [align=left] {\begin{minipage}[lt]{26.52pt}\setlength\topsep{0pt}
\begin{center}
\textbf{{\footnotesize Value}}
\end{center}

\end{minipage}};
% Text Node
\draw (430.5,149.25) node   [align=left] {\begin{minipage}[lt]{26.52pt}\setlength\topsep{0pt}
\begin{center}
\textbf{{\footnotesize Query}}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 202; green, 207; blue, 133 }  ,fill opacity=1 ][line width=1.5]   (272,282.25) -- (415,282.25) -- (415,315.25) -- (272,315.25) -- cycle  ;
\draw (343.5,298.75) node   [align=left] {\begin{minipage}[lt]{94.52pt}\setlength\topsep{0pt}
\begin{center}
\textbf{{\small Add \& Norm}}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 202; green, 207; blue, 133 }  ,fill opacity=1 ][line width=1.5]   (272,57.25) -- (415,57.25) -- (415,90.25) -- (272,90.25) -- cycle  ;
\draw (343.5,73.75) node   [align=left] {\begin{minipage}[lt]{94.52pt}\setlength\topsep{0pt}
\begin{center}
\textbf{{\small Add \& Norm}}
\end{center}

\end{minipage}};


\end{tikzpicture}


==> images/adversarial_fusion_phase1.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[rounded corners, x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,609); %set diagram left start at 0, and has height of 609

%Rounded Rect [id:dp6341074442210013] 
\draw  [fill={rgb, 255:red, 248; green, 247; blue, 255 }  ,fill opacity=1 ][line width=1.5]  (158,94.41) .. controls (158,68.23) and (179.23,47) .. (205.41,47) -- (484.59,47) .. controls (510.77,47) and (532,68.23) .. (532,94.41) -- (532,476.59) .. controls (532,502.77) and (510.77,524) .. (484.59,524) -- (205.41,524) .. controls (179.23,524) and (158,502.77) .. (158,476.59) -- cycle ;
%Straight Lines [id:da6825529649685187] 
\draw [color={rgb, 255:red, 70; green, 35; blue, 35 }  ,draw opacity=1 ][line width=1.5]    (345,538) -- (345,488.5) ;
\draw [shift={(345,484.5)}, rotate = 90] [fill={rgb, 255:red, 70; green, 35; blue, 35 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Curve Lines [id:da6217683049674494] 
\draw [color={rgb, 255:red, 70; green, 35; blue, 35 }  ,draw opacity=1 ][line width=1.5]    (322.06,484.27) .. controls (322.63,502.51) and (327.33,512.18) .. (345,511.25) .. controls (362.86,510.31) and (365.7,503.85) .. (365.98,484.8) ;
\draw [shift={(366,481)}, rotate = 90] [fill={rgb, 255:red, 70; green, 35; blue, 35 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
\draw [shift={(322,480)}, rotate = 90] [fill={rgb, 255:red, 70; green, 35; blue, 35 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da5002170436089142] 
\draw [color={rgb, 255:red, 70; green, 35; blue, 35 }  ,draw opacity=1 ][line width=2.25]    (345,428.5) -- (345,457) ;
%Straight Lines [id:da9185526315200156] 
\draw [color={rgb, 255:red, 70; green, 35; blue, 35 }  ,draw opacity=1 ][line width=2.25]    (345,366.5) -- (345,395.5) ;
%Straight Lines [id:da39192677265440934] 
\draw [color={rgb, 255:red, 70; green, 35; blue, 35 }  ,draw opacity=1 ][line width=2.25]    (345,310.5) -- (345,344) ;
%Straight Lines [id:da14362367551663113] 
\draw [color={rgb, 255:red, 70; green, 35; blue, 35 }  ,draw opacity=1 ][line width=1.5]  [dash pattern={on 1.69pt off 2.76pt}]  (345,164) -- (345,221.5) ;
\draw [shift={(345,160)}, rotate = 90] [fill={rgb, 255:red, 70; green, 35; blue, 35 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da25263190701138005] 
\draw [color={rgb, 255:red, 70; green, 35; blue, 35 }  ,draw opacity=1 ][line width=1.5]    (356,164.5) -- (356,191.5) -- (463,191.5) -- (463,236) ;
\draw [shift={(356,160.5)}, rotate = 90] [fill={rgb, 255:red, 70; green, 35; blue, 35 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da2916586528074192] 
\draw [color={rgb, 255:red, 70; green, 35; blue, 35 }  ,draw opacity=1 ][line width=2.25]    (345,327.25) -- (429,327.25) -- (429,163.5) ;
\draw [shift={(429,158.5)}, rotate = 90] [fill={rgb, 255:red, 70; green, 35; blue, 35 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;
%Straight Lines [id:da4003464351839461] 
\draw [line width=2.25]    (344,90.5) -- (344,108.5) ;
%Straight Lines [id:da10558611028169751] 
\draw [line width=2.25]    (344,35) -- (344,60.5) ;
\draw [shift={(344,30)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;
%Straight Lines [id:da7645130716911561] 
\draw [color={rgb, 255:red, 70; green, 35; blue, 35 }  ,draw opacity=1 ][line width=1.5]  [dash pattern={on 1.69pt off 2.76pt}]  (345,255) -- (345,285.5) ;
\draw [shift={(345,251)}, rotate = 90] [fill={rgb, 255:red, 70; green, 35; blue, 35 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da014364346306787734] 
\draw [color={rgb, 255:red, 70; green, 35; blue, 35 }  ,draw opacity=1 ][line width=1.5]    (334,164.5) -- (334,191.5) -- (220,191.5) -- (220,226) ;
\draw [shift={(334,160.5)}, rotate = 90] [fill={rgb, 255:red, 70; green, 35; blue, 35 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da6829981786866541] 
\draw [color={rgb, 255:red, 70; green, 35; blue, 35 }  ,draw opacity=1 ][line width=1.5]    (262,164.5) -- (262,191.5) -- (220,191.5) -- (220,226) ;
\draw [shift={(262,160.5)}, rotate = 90] [fill={rgb, 255:red, 70; green, 35; blue, 35 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da9001010049945131] 
\draw [color={rgb, 255:red, 70; green, 35; blue, 35 }  ,draw opacity=1 ][line width=1.5]  [dash pattern={on 1.69pt off 2.76pt}]  (270,165) -- (270,199.5) -- (345,199.5) -- (345,221.5) ;
\draw [shift={(270,161)}, rotate = 90] [fill={rgb, 255:red, 70; green, 35; blue, 35 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da21521766310937984] 
\draw [color={rgb, 255:red, 70; green, 35; blue, 35 }  ,draw opacity=1 ][line width=1.5]    (279,165) -- (279,206.5) -- (463,206) -- (463,231) ;
\draw [shift={(279,161)}, rotate = 90] [fill={rgb, 255:red, 70; green, 35; blue, 35 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da5876432184676101] 
\draw [color={rgb, 255:red, 70; green, 35; blue, 35 }  ,draw opacity=1 ][line width=1.5]    (220,255) -- (220,272) -- (345,272.5) -- (345,301.5) ;
\draw [shift={(220,251)}, rotate = 90] [fill={rgb, 255:red, 70; green, 35; blue, 35 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da12410819983578247] 
\draw [color={rgb, 255:red, 70; green, 35; blue, 35 }  ,draw opacity=1 ][line width=1.5]    (462,255) -- (462,272) -- (345,272.5) -- (345,301.5) ;
\draw [shift={(462,251)}, rotate = 90] [fill={rgb, 255:red, 70; green, 35; blue, 35 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;

% Text Node
\draw  [fill={rgb, 255:red, 255; green, 172; blue, 129 }  ,fill opacity=1 ][line width=2.25]   (255.5,451.5) -- (430.5,451.5) -- (430.5,484.5) -- (255.5,484.5) -- cycle  ;
\draw (343,468) node   [align=left] {\begin{minipage}[lt]{116.28pt}\setlength\topsep{0pt}
\begin{center}
{\small \textbf{Multi-Head Attention}}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 202; green, 207; blue, 133 }  ,fill opacity=1 ][line width=1.5]   (270,396.25) -- (417,396.25) -- (417,429.25) -- (270,429.25) -- cycle  ;
\draw (343.5,412.75) node   [align=left] {\begin{minipage}[lt]{97.24pt}\setlength\topsep{0pt}
\begin{center}
\textbf{{\small Add \& Norm}}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 77; green, 179; blue, 252 }  ,fill opacity=1 ][line width=2.25]   (257,339.75) -- (429,339.75) -- (429,372.75) -- (257,372.75) -- cycle  ;
\draw (343,356.25) node   [align=left] {\begin{minipage}[lt]{114.24pt}\setlength\topsep{0pt}
\begin{center}
\textbf{{\small Feed Forward }}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 128; green, 147; blue, 241 }  ,fill opacity=1 ][line width=2.25]   (410.5,218.5) -- (515.5,218.5) -- (515.5,253.5) -- (410.5,253.5) -- cycle  ;
\draw (463,236) node   [align=left] {\begin{minipage}[lt]{68.68pt}\setlength\topsep{0pt}
\begin{center}
{\small \textbf{Lang}\textsubscript{\textbf{n}}\textbf{ Adapter}}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 154; green, 189; blue, 151 }  ,fill opacity=1 ][line width=1.5]   (213,109.5) -- (464,109.5) -- (464,161.5) -- (213,161.5) -- cycle  ;
\draw (338.5,135.5) node   [align=left] {\begin{minipage}[lt]{167.96pt}\setlength\topsep{0pt}
\begin{center}
\textbf{{\small {\fontfamily{helvet}\selectfont AdvFusion Adapter }}}
\end{center}

\end{minipage}};
% Text Node
\draw (270.5,148.25) node   [align=left] {\begin{minipage}[lt]{26.52pt}\setlength\topsep{0pt}
\begin{center}
\textbf{{\footnotesize Key}}
\end{center}

\end{minipage}};
% Text Node
\draw (345.5,149.25) node   [align=left] {\begin{minipage}[lt]{26.52pt}\setlength\topsep{0pt}
\begin{center}
\textbf{{\footnotesize Value}}
\end{center}

\end{minipage}};
% Text Node
\draw (426.5,149.25) node   [align=left] {\begin{minipage}[lt]{26.52pt}\setlength\topsep{0pt}
\begin{center}
\textbf{{\footnotesize Query}}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 202; green, 207; blue, 133 }  ,fill opacity=1 ][line width=1.5]   (270,282.25) -- (417,282.25) -- (417,315.25) -- (270,315.25) -- cycle  ;
\draw (343.5,298.75) node   [align=left] {\begin{minipage}[lt]{97.24pt}\setlength\topsep{0pt}
\begin{center}
\textbf{{\small Add \& Norm}}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 202; green, 207; blue, 133 }  ,fill opacity=1 ][line width=1.5]   (274,59.25) -- (417,59.25) -- (417,92.25) -- (274,92.25) -- cycle  ;
\draw (345.5,75.75) node   [align=left] {\begin{minipage}[lt]{94.52pt}\setlength\topsep{0pt}
\begin{center}
\textbf{{\small Add \& Norm}}
\end{center}

\end{minipage}};
% Text Node
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=0.52 ][fill={rgb, 255:red, 128; green, 147; blue, 241 }  ,fill opacity=1 ][dash pattern={on 5.63pt off 4.5pt}][line width=1.5]   (292,218.5) -- (398,218.5) -- (398,254.5) -- (292,254.5) -- cycle  ;
\draw (345,236.5) node  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=0.54 ] [align=left] {\begin{minipage}[lt]{69.36pt}\setlength\topsep{0pt}
\begin{center}
{\small \textbf{Lang}\textsubscript{\textbf{k}}\textbf{ Adapter}}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 128; green, 147; blue, 241 }  ,fill opacity=1 ][line width=2.25]   (169.75,218.5) -- (279.75,218.5) -- (279.75,254.5) -- (169.75,254.5) -- cycle  ;
\draw (224.75,236.5) node   [align=left] {\begin{minipage}[lt]{71.74pt}\setlength\topsep{0pt}
\begin{center}
{\small \textbf{Lang}\textsubscript{\textbf{1}}\textbf{ Adapter }}
\end{center}

\end{minipage}};


\end{tikzpicture}

==> images/adversarial_fusion_phase2.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[rounded corners, x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,609); %set diagram left start at 0, and has height of 609

%Rounded Rect [id:dp03992242326373008] 
\draw  [fill={rgb, 255:red, 248; green, 247; blue, 255 }  ,fill opacity=1 ][line width=1.5]  (178,114.41) .. controls (178,88.23) and (199.23,67) .. (225.41,67) -- (504.59,67) .. controls (530.77,67) and (552,88.23) .. (552,114.41) -- (552,496.59) .. controls (552,522.77) and (530.77,544) .. (504.59,544) -- (225.41,544) .. controls (199.23,544) and (178,522.77) .. (178,496.59) -- cycle ;
%Straight Lines [id:da04315805775251569] 
\draw [color={rgb, 255:red, 70; green, 35; blue, 35 }  ,draw opacity=1 ][line width=1.5]    (365,558) -- (365,508.5) ;
\draw [shift={(365,504.5)}, rotate = 90] [fill={rgb, 255:red, 70; green, 35; blue, 35 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Curve Lines [id:da24612668073333976] 
\draw [color={rgb, 255:red, 70; green, 35; blue, 35 }  ,draw opacity=1 ][line width=1.5]    (342.06,504.27) .. controls (342.63,522.51) and (347.33,532.18) .. (365,531.25) .. controls (382.86,530.31) and (385.7,523.85) .. (385.98,504.8) ;
\draw [shift={(386,501)}, rotate = 90] [fill={rgb, 255:red, 70; green, 35; blue, 35 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
\draw [shift={(342,500)}, rotate = 90] [fill={rgb, 255:red, 70; green, 35; blue, 35 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da5891583724247711] 
\draw [color={rgb, 255:red, 70; green, 35; blue, 35 }  ,draw opacity=1 ][line width=2.25]    (365,448.5) -- (365,477) ;
%Straight Lines [id:da9719258924038408] 
\draw [color={rgb, 255:red, 70; green, 35; blue, 35 }  ,draw opacity=1 ][line width=2.25]    (365,386.5) -- (365,415.5) ;
%Straight Lines [id:da11356680983173972] 
\draw [color={rgb, 255:red, 70; green, 35; blue, 35 }  ,draw opacity=1 ][line width=2.25]    (365,330.5) -- (365,364) ;
%Straight Lines [id:da17222056250514006] 
\draw [color={rgb, 255:red, 70; green, 35; blue, 35 }  ,draw opacity=1 ][line width=1.5]    (365,184) -- (365,241.5) ;
\draw [shift={(365,180)}, rotate = 90] [fill={rgb, 255:red, 70; green, 35; blue, 35 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da5029919975206567] 
\draw [color={rgb, 255:red, 70; green, 35; blue, 35 }  ,draw opacity=1 ][line width=1.5]    (376,184.5) -- (376,211.5) -- (483,211.5) -- (483,256) ;
\draw [shift={(376,180.5)}, rotate = 90] [fill={rgb, 255:red, 70; green, 35; blue, 35 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da36073827023882177] 
\draw [color={rgb, 255:red, 70; green, 35; blue, 35 }  ,draw opacity=1 ][line width=2.25]    (365,347.25) -- (449,347.25) -- (449,183.5) ;
\draw [shift={(449,178.5)}, rotate = 90] [fill={rgb, 255:red, 70; green, 35; blue, 35 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;
%Straight Lines [id:da3059100596241533] 
\draw [line width=2.25]    (364,110.5) -- (364,128.5) ;
%Straight Lines [id:da17885139572983388] 
\draw [line width=2.25]    (364,55) -- (364,80.5) ;
\draw [shift={(364,50)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;
%Straight Lines [id:da9979265466700413] 
\draw [color={rgb, 255:red, 70; green, 35; blue, 35 }  ,draw opacity=1 ][line width=1.5]  [dash pattern={on 1.69pt off 2.76pt}]  (365,275) -- (365,305.5) ;
\draw [shift={(365,271)}, rotate = 90] [fill={rgb, 255:red, 70; green, 35; blue, 35 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da1958347412646182] 
\draw [color={rgb, 255:red, 70; green, 35; blue, 35 }  ,draw opacity=1 ][line width=1.5]    (354,184.5) -- (354,211.5) -- (240,211.5) -- (240,246) ;
\draw [shift={(354,180.5)}, rotate = 90] [fill={rgb, 255:red, 70; green, 35; blue, 35 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da4623363888857679] 
\draw [color={rgb, 255:red, 70; green, 35; blue, 35 }  ,draw opacity=1 ][line width=1.5]    (282,184.5) -- (282,211.5) -- (240,211.5) -- (240,246) ;
\draw [shift={(282,180.5)}, rotate = 90] [fill={rgb, 255:red, 70; green, 35; blue, 35 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da4476042049637312] 
\draw [color={rgb, 255:red, 70; green, 35; blue, 35 }  ,draw opacity=1 ][line width=1.5]    (290,185) -- (290,219.5) -- (365,219.5) -- (365,241.5) ;
\draw [shift={(290,181)}, rotate = 90] [fill={rgb, 255:red, 70; green, 35; blue, 35 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da43131118018930925] 
\draw [color={rgb, 255:red, 70; green, 35; blue, 35 }  ,draw opacity=1 ][line width=1.5]    (299,185) -- (299,226.5) -- (483,226) -- (483,251) ;
\draw [shift={(299,181)}, rotate = 90] [fill={rgb, 255:red, 70; green, 35; blue, 35 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da9872683138852032] 
\draw [color={rgb, 255:red, 70; green, 35; blue, 35 }  ,draw opacity=1 ][line width=1.5]    (240,275) -- (240,292) -- (365,292.5) -- (365,321.5) ;
\draw [shift={(240,271)}, rotate = 90] [fill={rgb, 255:red, 70; green, 35; blue, 35 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da1144277526120685] 
\draw [color={rgb, 255:red, 70; green, 35; blue, 35 }  ,draw opacity=1 ][line width=1.5]    (482,275) -- (482,292) -- (365,292.5) -- (365,321.5) ;
\draw [shift={(482,271)}, rotate = 90] [fill={rgb, 255:red, 70; green, 35; blue, 35 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;

% Text Node
\draw  [fill={rgb, 255:red, 255; green, 172; blue, 129 }  ,fill opacity=1 ][line width=2.25]   (275.5,471.5) -- (450.5,471.5) -- (450.5,504.5) -- (275.5,504.5) -- cycle  ;
\draw (363,488) node   [align=left] {\begin{minipage}[lt]{116.28pt}\setlength\topsep{0pt}
\begin{center}
{\small \textbf{Multi-Head Attention}}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 202; green, 207; blue, 133 }  ,fill opacity=1 ][line width=1.5]   (290,416.25) -- (437,416.25) -- (437,449.25) -- (290,449.25) -- cycle  ;
\draw (363.5,432.75) node   [align=left] {\begin{minipage}[lt]{97.24pt}\setlength\topsep{0pt}
\begin{center}
\textbf{{\small Add \& Norm}}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 77; green, 179; blue, 252 }  ,fill opacity=1 ][line width=2.25]   (277,359.75) -- (449,359.75) -- (449,392.75) -- (277,392.75) -- cycle  ;
\draw (363,376.25) node   [align=left] {\begin{minipage}[lt]{114.24pt}\setlength\topsep{0pt}
\begin{center}
\textbf{{\small Feed Forward }}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 128; green, 147; blue, 241 }  ,fill opacity=1 ][line width=2.25]   (430.5,238.5) -- (535.5,238.5) -- (535.5,273.5) -- (430.5,273.5) -- cycle  ;
\draw (483,256) node   [align=left] {\begin{minipage}[lt]{68.68pt}\setlength\topsep{0pt}
\begin{center}
{\small \textbf{Lang}\textsubscript{\textbf{n}}\textbf{ Adapter}}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 154; green, 189; blue, 151 }  ,fill opacity=1 ][line width=1.5]   (233,129.5) -- (484,129.5) -- (484,181.5) -- (233,181.5) -- cycle  ;
\draw (358.5,155.5) node   [align=left] {\begin{minipage}[lt]{167.96pt}\setlength\topsep{0pt}
\begin{center}
\textbf{{\small {\fontfamily{helvet}\selectfont AdvFusion Adapter }}}
\end{center}

\end{minipage}};
% Text Node
\draw (290.5,168.25) node   [align=left] {\begin{minipage}[lt]{26.52pt}\setlength\topsep{0pt}
\begin{center}
\textbf{{\footnotesize Key}}
\end{center}

\end{minipage}};
% Text Node
\draw (365.5,169.25) node   [align=left] {\begin{minipage}[lt]{26.52pt}\setlength\topsep{0pt}
\begin{center}
\textbf{{\footnotesize Value}}
\end{center}

\end{minipage}};
% Text Node
\draw (446.5,169.25) node   [align=left] {\begin{minipage}[lt]{26.52pt}\setlength\topsep{0pt}
\begin{center}
\textbf{{\footnotesize Query}}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 202; green, 207; blue, 133 }  ,fill opacity=1 ][line width=1.5]   (290,302.25) -- (437,302.25) -- (437,335.25) -- (290,335.25) -- cycle  ;
\draw (363.5,318.75) node   [align=left] {\begin{minipage}[lt]{97.24pt}\setlength\topsep{0pt}
\begin{center}
\textbf{{\small Add \& Norm}}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 202; green, 207; blue, 133 }  ,fill opacity=1 ][line width=1.5]   (294,79.25) -- (437,79.25) -- (437,112.25) -- (294,112.25) -- cycle  ;
\draw (365.5,95.75) node   [align=left] {\begin{minipage}[lt]{94.52pt}\setlength\topsep{0pt}
\begin{center}
\textbf{{\small Add \& Norm}}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 128; green, 147; blue, 241 }  ,fill opacity=1 ][line width=2.25]   (189.75,238.5) -- (299.75,238.5) -- (299.75,274.5) -- (189.75,274.5) -- cycle  ;
\draw (244.75,256.5) node   [align=left] {\begin{minipage}[lt]{71.74pt}\setlength\topsep{0pt}
\begin{center}
{\small \textbf{Lang}\textsubscript{\textbf{1}}\textbf{ Adapter }}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 128; green, 147; blue, 241 }  ,fill opacity=1 ][line width=2.25]   (312,238.5) -- (417,238.5) -- (417,273.5) -- (312,273.5) -- cycle  ;
\draw (364.5,256) node   [align=left] {\begin{minipage}[lt]{68.68pt}\setlength\topsep{0pt}
\begin{center}
{\small \textbf{Lang}\textsubscript{k}\textbf{ Adapter}}
\end{center}

\end{minipage}};


\end{tikzpicture}


==> images/internal_fusion.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[rounded corners,x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,495); %set diagram left start at 0, and has height of 495

%Rounded Rect [id:dp13798027349488695] 
\draw  [fill={rgb, 255:red, 183; green, 220; blue, 155 }  ,fill opacity=1 ][line width=1.5]  (168,89) .. controls (168,80.16) and (175.16,73) .. (184,73) -- (449,73) .. controls (457.84,73) and (465,80.16) .. (465,89) -- (465,215) .. controls (465,223.84) and (457.84,231) .. (449,231) -- (184,231) .. controls (175.16,231) and (168,223.84) .. (168,215) -- cycle ;
%Straight Lines [id:da7977539392701258] 
\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (228,305.5) -- (317,305.5) -- (317,220) ;
\draw [shift={(317,216)}, rotate = 90] [fill={rgb, 255:red, 74; green, 74; blue, 74 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da8650824443043985] 
\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (231,305.5) -- (299,305.5) -- (299,221) ;
\draw [shift={(299,217)}, rotate = 90] [fill={rgb, 255:red, 74; green, 74; blue, 74 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da7309864536263377] 
\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (189,265) -- (189,219) ;
\draw [shift={(189,215)}, rotate = 90] [fill={rgb, 255:red, 74; green, 74; blue, 74 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da09341468421889854] 
\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (207,265) -- (207,219) ;
\draw [shift={(207,215)}, rotate = 90] [fill={rgb, 255:red, 74; green, 74; blue, 74 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Rounded Rect [id:dp732628763486608] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=0.3 ][fill={rgb, 255:red, 147; green, 185; blue, 229 }  ,fill opacity=0.29 ][line width=1.5]  (139.42,287.16) .. controls (139.42,279.11) and (145.95,272.58) .. (154,272.58) -- (289.84,272.58) .. controls (297.89,272.58) and (304.42,279.11) .. (304.42,287.16) -- (304.42,402) .. controls (304.42,410.05) and (297.89,416.58) .. (289.84,416.58) -- (154,416.58) .. controls (145.95,416.58) and (139.42,410.05) .. (139.42,402) -- cycle ;
%Rounded Rect [id:dp07457754772974523] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=0.5 ][fill={rgb, 255:red, 147; green, 185; blue, 229 }  ,fill opacity=0.54 ][line width=1.5]  (146.42,280.16) .. controls (146.42,272.11) and (152.95,265.58) .. (161,265.58) -- (296.84,265.58) .. controls (304.89,265.58) and (311.42,272.11) .. (311.42,280.16) -- (311.42,395) .. controls (311.42,403.05) and (304.89,409.58) .. (296.84,409.58) -- (161,409.58) .. controls (152.95,409.58) and (146.42,403.05) .. (146.42,395) -- cycle ;
%Straight Lines [id:da5424628992319724] 
\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (190,434) -- (190,416) ;
%Straight Lines [id:da7816652142982661] 
\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (209,431) -- (209,409) ;
%Straight Lines [id:da42229231795943467] 
\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (189,191.5) -- (189,95) -- (302,95) ;
\draw [shift={(306,95)}, rotate = 180] [fill={rgb, 255:red, 74; green, 74; blue, 74 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da5993146615121212] 
\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (209,191.5) -- (209,95) -- (303,95) ;
\draw [shift={(307,95)}, rotate = 180] [fill={rgb, 255:red, 74; green, 74; blue, 74 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da39329061235196194] 
\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (228,191.5) -- (228,95) -- (302,95) ;
\draw [shift={(306,95)}, rotate = 180] [fill={rgb, 255:red, 74; green, 74; blue, 74 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da11961534053205458] 
\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (298,199.5) -- (298,182) -- (309.07,171.72) ;
\draw [shift={(312,169)}, rotate = 137.12] [fill={rgb, 255:red, 74; green, 74; blue, 74 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da7226753607828844] 
\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (334,196.5) -- (334,180) -- (322.23,171.37) ;
\draw [shift={(319,169)}, rotate = 36.25] [fill={rgb, 255:red, 74; green, 74; blue, 74 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da4186963494050291] 
\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (315.5,193) -- (315.91,175) ;
\draw [shift={(316,171)}, rotate = 91.3] [fill={rgb, 255:red, 74; green, 74; blue, 74 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da5030376724541119] 
\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (316.5,151.13) -- (316.5,142) ;
%Straight Lines [id:da748685871072964] 
\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (422,191.5) -- (422,158) -- (332,158) ;
\draw [shift={(328,158)}, rotate = 360] [fill={rgb, 255:red, 74; green, 74; blue, 74 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da3401197506323823] 
\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (316.5,118.13) -- (316.5,103) ;
%Straight Lines [id:da16197390471731854] 
\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (316.5,84) -- (316.5,60) ;
\draw [shift={(316.5,56)}, rotate = 90] [fill={rgb, 255:red, 74; green, 74; blue, 74 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Rounded Rect [id:dp25424533271040173] 
\draw  [fill={rgb, 255:red, 147; green, 185; blue, 229 }  ,fill opacity=1 ][line width=1.5]  (154,272.58) .. controls (154,264.53) and (160.53,258) .. (168.58,258) -- (304.42,258) .. controls (312.47,258) and (319,264.53) .. (319,272.58) -- (319,387.42) .. controls (319,395.47) and (312.47,402) .. (304.42,402) -- (168.58,402) .. controls (160.53,402) and (154,395.47) .. (154,387.42) -- cycle ;
%Straight Lines [id:da7930110173721745] 
\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (228,266) -- (228,220) ;
\draw [shift={(228,216)}, rotate = 90] [fill={rgb, 255:red, 74; green, 74; blue, 74 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da6236989267199802] 
\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (228,314) -- (228,291) ;
\draw [shift={(228,287)}, rotate = 90] [fill={rgb, 255:red, 74; green, 74; blue, 74 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da7565752539778166] 
\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (229,352) -- (229,335) ;
\draw [shift={(229,331)}, rotate = 90] [fill={rgb, 255:red, 74; green, 74; blue, 74 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da5190979095996715] 
\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (229,430) -- (229,374) ;
\draw [shift={(229,370)}, rotate = 90] [fill={rgb, 255:red, 74; green, 74; blue, 74 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da5326935443569123] 
\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (211,490) -- (211,462) ;
\draw [shift={(211,458)}, rotate = 90] [fill={rgb, 255:red, 74; green, 74; blue, 74 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da5245538006673764] 
\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (317.5,28) -- (317.5,4) ;
\draw [shift={(317.5,0)}, rotate = 90] [fill={rgb, 255:red, 74; green, 74; blue, 74 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da5723990069061562] 
\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (228,305.5) -- (334,305.5) -- (334,219) ;
\draw [shift={(334,215)}, rotate = 90] [fill={rgb, 255:red, 74; green, 74; blue, 74 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da07174046750517515] 
\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (211,476.5) -- (424,476.5) -- (424,221) ;
\draw [shift={(424,217)}, rotate = 90] [fill={rgb, 255:red, 74; green, 74; blue, 74 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da17262823424253582] 
\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (132,490) -- (132,42) -- (257,42) ;
\draw [shift={(261,42)}, rotate = 180] [fill={rgb, 255:red, 74; green, 74; blue, 74 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;

% Text Node
\draw (403,83.75) node   [align=left] {\begin{minipage}[lt]{116.28pt}\setlength\topsep{0pt}
\begin{center}
\textbf{{\small Adapter Fusion }}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 213; green, 148; blue, 226 }  ,fill opacity=1 ][line width=1.5]   (180,192.18) -- (247,192.18) -- (247,217.18) -- (180,217.18) -- cycle  ;
\draw (213.5,204.68) node   [align=left] {\begin{minipage}[lt]{42.84pt}\setlength\topsep{0pt}
\begin{center}
value
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 126; green, 168; blue, 218 }  ,fill opacity=1 ][line width=1.5]   (283,192.18) -- (351,192.18) -- (351,217.18) -- (283,217.18) -- cycle  ;
\draw (317,204.68) node   [align=left] {\begin{minipage}[lt]{43.52pt}\setlength\topsep{0pt}
\begin{center}
key
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ][line width=1.5]   (283,117) -- (352,117) -- (352,143) -- (283,143) -- cycle  ;
\draw (317.5,130) node   [align=left] {\begin{minipage}[lt]{44.2pt}\setlength\topsep{0pt}
\begin{center}
softmax
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 230; green, 197; blue, 142 }  ,fill opacity=1 ][line width=1.5]   (387,192.18) -- (454,192.18) -- (454,217.18) -- (387,217.18) -- cycle  ;
\draw (420.5,204.68) node   [align=left] {\begin{minipage}[lt]{42.84pt}\setlength\topsep{0pt}
\begin{center}
query
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ][line width=1.5]   (263,29) -- (368,29) -- (368,55) -- (263,55) -- cycle  ;
\draw (315.5,42) node   [align=left] {\begin{minipage}[lt]{68.68pt}\setlength\topsep{0pt}
\begin{center}
add \& norm
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 213; green, 225; blue, 240 }  ,fill opacity=1 ][line width=1.5]   (317, 161.5) circle [x radius= 11.31, y radius= 10.61]   ;
\draw (317,161.5) node   [align=left] {\begin{minipage}[lt]{10.88pt}\setlength\topsep{0pt}
\begin{center}
{\large ×}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 213; green, 225; blue, 240 }  ,fill opacity=1 ][line width=1.5]   (316, 93.5) circle [x radius= 11.31, y radius= 10.61]   ;
\draw (316,93.5) node   [align=left] {\begin{minipage}[lt]{10.88pt}\setlength\topsep{0pt}
\begin{center}
{\large ×}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 213; green, 225; blue, 240 }  ,fill opacity=1 ][line width=1.5]   (228, 276.5) circle [x radius= 11.31, y radius= 10.61]   ;
\draw (228,276.5) node   [align=left] {\begin{minipage}[lt]{10.88pt}\setlength\topsep{0pt}
\begin{center}
{\large ×}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ][line width=1.5]   (179,313.09) -- (278,313.09) -- (278,331.09) -- (179,331.09) -- cycle  ;
\draw (228.5,322.09) node   [align=left] {\begin{minipage}[lt]{64.6pt}\setlength\topsep{0pt}
\begin{center}
{\small FF Up}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ][line width=1.5]   (179,351.09) -- (278,351.09) -- (278,369.09) -- (179,369.09) -- cycle  ;
\draw (228.5,360.09) node   [align=left] {\begin{minipage}[lt]{64.6pt}\setlength\topsep{0pt}
\begin{center}
{\small FF Down}
\end{center}

\end{minipage}};
% Text Node
\draw (283.29,272.58) node   [align=left] {\begin{minipage}[lt]{49.92pt}\setlength\topsep{0pt}
\begin{center}
\textbf{{\footnotesize Language}}\\\textbf{{\footnotesize Adapters}}
\end{center}
\end{minipage}};


% Text Node
\draw  [fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ][line width=1.5]   (163,431) -- (268,431) -- (268,457) -- (163,457) -- cycle  ;
\draw (215.5,444) node   [align=left] {\begin{minipage}[lt]{68.68pt}\setlength\topsep{0pt}
\begin{center}
add \& norm
\end{center}

\end{minipage}};


\end{tikzpicture}

